Efficient Self-supervised Vision Transformers for Representation Learning

This paper investigates two techniques for developing efficient self-supervised vision transformers (EsViT) for visual representation learning. First, we show through a comprehensive empirical study that multi-stage architectures with sparse self-attentions can significantly reduce modeling complexity but with a cost of losing the ability to capture fine-grained correspondences between image regions. Second, we propose a new pre-training task of region matching which allows the model to capture fine-grained region dependencies and as a result significantly improves the quality of the learned vision representations. Our results show that combining the two techniques, EsViT achieves 81.3% top-1 on the ImageNet linear probe evaluation, outperforming prior arts with around an order magnitude of higher throughput. When transferring to downstream linear classification tasks, EsViT outperforms its supervised counterpart on 17 out of 18 datasets. The code and models are publicly available: https://github.com/microsoft/esvit

==> subtex/checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~?.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{In abstract and introduction, we present EsViT, by considering a multi-stage architecture and a region-based pre-training task for self-supervised Transformers.}
  \item Did you describe the limitations of your work?
    \answerYes{We point out several limitations in Section 4, when comparing the experimental results with some existing works.}  
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section 4 and Appendix B.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{In our experiments, we either fix hyper-parameters by following existing works, or report the best results, after sweeping a range of hyper-parameter values as suggested in previous works.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
     \answerYes{See Section 4 and Appendix B.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> subtex/main_arxiv.tex <==
\maketitle

\begin{abstract}
  
%  This paper investigates efficient self-supervised vision transformers (\shortname{}) for visual representation learning. The first empirical study is presented on multi-stage ViT architectures for self-supervised learning. 
%  Our study reveals two insights towards building \shortname{}:
%  1) Multi-stage architectures with sparse self-attentions can greatly reduce complexity, but lacks correspondences between regions.
%  2) A region matching pre-training task is proposed to improve the efficiency and boost learned representations significantly.
This paper investigates two techniques for developing efficient self-supervised vision transformers (\shortname{}) for visual representation learning. First, we show through a comprehensive empirical study that multi-stage architectures with sparse self-attentions can significantly reduce modeling complexity but with a cost of losing the ability to capture fine-grained correspondences between image regions. Second, we propose a new pre-training task of region matching which allows the model to capture fine-grained region dependencies and as a result significantly improves the quality of the learned vision representations. 
%We show that the synergy of both in 
Our results show that combining the two techniques, \shortname{} achieves 81.3\% top-1 accuracy on the ImageNet linear probe evaluation, outperforming prior arts with around an order magnitude of higher throughput.  When transferring to downstream linear classification tasks, \shortname{} outperforms its supervised counterpart on 17 out of 18 datasets.
The code and models will be publicly available.   

%   \JG{Do you position the paper as an empirical study or to propose a new method -- EsViT? If it is both, then clarify that ``we first present an empirical study..., Then, we propose a new region-level pre-training task (MPP) inspired by MLM for language model pre-training to significantly improve the efficiency of SSL of vision transformers, leading to new SoTA results on...''}
  

\end{abstract}

%   Region-mixed data augmentations help when added in the late stage of pre-training.

\section{Introduction}
\vspace{-2mm}
Self-supervised learning (SSL) with Transformers~\citep{vaswani2017attention} has become a de facto standard of model choice in natural language processing (NLP). The dominant approaches such as GPT~\citep{radford2018improving} and BERT~\citep{devlin2019bert} are pre-training on a large text corpus and then fine-tuning to various smaller task-specific datasets, showing superior performance. Larger Transformers pre-trained with larger-scale language datasets often lead to a stronger generalization ability, demonstrated by improved performance in downsteam tasks (with no sign of performance saturation yet), as exemplified in GPT-3~\citep{brown2020language}. 

In computer vision (CV), however, self-supervised visual representation learning is still dominated by convolutional neural networks (CNNs). Sharing a similar goal/spirit with NLP, SSL in CV aims to learn general-purpose image features from raw pixels without relying on manual supervisions, and the learned networks are expected to serve as the backbone of various downstream tasks such as classification, detection and segmentation. Recently, impressive performance have been achieved by CNN-based SSL, outperforming state-of-the-art (SoTA) fully-supervised pre-training methods~\citep{he2020momentum,caron2020unsupervised} on tasks with a limited number of labels. The key to success is view-level learning: maximizing agreement of learned representations between differently augmented views of the same example.  Recent works, including SimCLR-v2~\citep{chen2020big}, BYOL~\citep{grill2020bootstrap} and SwAV~\citep{caron2020unsupervised}, have scaled up the CNN-based models to hundreds of millions of parameters.
However, SSL has not enjoyed the same scaling success in CV as that in NLP.
%However, a large performance gap remains for CNN-based SSL in CV, 
% compared to the success of Transformers in NLP. However, despite the success of Transformers in NLP, a big performance gap between Transformer-based SSL and CNN-based SSL remains in CV.

 
% and is becoming the building block in many computer vision applications. 

% The pre-trained model produces general-purpose features and serve as the backbone of various downstream tasks such as classification, detection and segmentation, improving the generalization of those task-specific models that are often trained on limited amounts of task labels. 

Several attempts have been made to close the gap by combining SSL with Transformer and self-attention architectures. Early works include Selfie~\citep{trinh2019selfie}, which generalizes the concept of masked language modeling of BERT for images. The idea has been recently revisited in Vision Transformer (ViT)~\citep{dosovitskiy2020image} via pre-training on a much larger scale dataset, \eg JFT-300M.  ImageGPT (iGPT)~\citep{chen2020generative} generalizes the concept of auto-regressive language modeling of GPT for images, showing encouraging ImageNet recognition accuracy with a large model size. Contrastive learning with ViT has also been studied very recently in DINO~\citep{caron2021emerging} and MoCo-v3~\citep{chen2021empirical}, where new SoTA result by  linear probe evaluation on ImageNet-1K is achieved, by exhaustively consuming computation resource on full self-attention operators with long sequences of split image patches.

% \begin{wrapfigure}{R}{0.45\textwidth}
% \vspace{-5mm}
% \begin{minipage}{0.55\textwidth}
% \scriptsize
% \centering
% \hspace{-3mm}
% \includegraphics[height=5.2cm]{figs/ssl_sota_tradeoff.pdf}
% \vspace{-1mm}
% \caption{\small Comparison under the linear classification protocol
% on ImageNet. All are reported as unsupervised pre-training on the ImageNet-1M training set, followed by supervised linear classification trained on frozen features, evaluated on the validation set. The parameter counts are those of the feature extractors.} 
% \label{fig:ssl_sota_curves}
% \vspace{-2mm}
% \end{minipage}
% \end{wrapfigure}


\begin{figure*}[t!]%\vspace{-25pt}
	\vspace{-0mm}\centering
	\begin{tabular}{c c}
		\hspace{-4mm}
		\includegraphics[height=4.55cm]{figs/ssl_sota_tradeoff_throughput.pdf}  & 
		% \vspace{2mm}
		\hspace{-0mm}
		\includegraphics[height=4.6cm]{figs/ssl_sota_tradeoff.pdf} \\
% 		(a) Proposed multi-stage architecture \vspace{2mm} & 
% 		\hspace{-6mm}
% 		(b) Baseline monolithic architecture \hspace{-0mm} \\ 
	\end{tabular}
	\vspace{-3mm}
	\caption{Efficiency vs accuracy comparison under the linear classification protocol on ImageNet. Left: Throughput of all SoTA SSL vision systems, circle sizes indicates model parameter counts; Right: performance over varied parameter counts for models with moderate (throughout/\#parameters) ratio. Please refer Section~\ref{sec:imagenet_probe} for details.
	 }
	\vspace{-5mm}
	\label{fig:hero_cmp}
\end{figure*}

% 	 \footnote{MoCo-v3 ViT/7 and DINO DeiT/8 are excluded when comparing model size, as they requires much higher compute complexity per parameter count than others, shown in Table~\ref{tab:main_result_cls}. }



Aiming to improve the {\em efficiency} of Transformer-based SSL, this paper presents {\em {\bf E}fficient {\bf s}elf-superivsed {\bf Vi}sion {\bf T}ransformers} (\shortname{}), by using a multi-stage architecture and a region-based pre-training task for self-supervised representation learning. 
Our main findings and contributions can be summarized as follows:

% \JG{I suggest you rewrite the main contributions based on abstract. e.g., (1) we conduct an empirical study to show the pros and cons of multi-scale architecture; (2) we propose a new pre-training task of region matching, (3) we validate the new EsViT, which combines the two tech, on a range of tasks, showing that...}

\begin{minipage}{1.0\textwidth}
\centering

\begin{itemize}[leftmargin=5.5mm]
\item  An intriguing property of self-supervised monolithic Transformers is firstly reported in our paper: automatic discovery of semantic correspondence between local regions. 

\item  We present the first comprehensive empirical study to show the pros and cons of multi-stage vision Transformer architectures for SSL. Though greatly reducing compute complexity, we find that the multi-stage architecture causes the loss of this property.  

\item 
A region matching pre-train task is proposed to alleviate this issue, and further improve the learned representations and attentions.

\item  
We validate the new \shortname{}, which combines the two techniques, on a range of tasks.
It significantly reduces the cost in building SoTA SSL vision systems, as summarized in Figure~\ref{fig:hero_cmp}, and shows better scaling performance on accuracy vs. throughput and model size.
Under the linear evaluation protocol, \shortname{} achieves 81.3\% top-1 accuracy, showing the best performance compared with all systems, and is $3.5\times$ parameter-efficient and has at least $10\times$ higher throughput than previous SoTA (81.0\%, MoCo-v3 with ViT-BN-L/7~\citep{chen2021empirical}). 
%
Compared with its supervised counterpart Swin Transformers~\citep{liu2021Swin}, \shortname{} shows superior performance on 17 out 18 datasets, when transferring the learned representations to downstream linear classification tasks. 

\end{itemize}

\end{minipage}



% ~\CL{To do in the end}
% We further investigate the impact of pre-training datasets and data augmentations, to set a solid baseline for future research in efficient Transformer-based SSL.
%

% $(\RN{1})$ 
% $(\RN{2})$ 
% $(\RN{3})$
% $(\RN{4})$



% The multi-stage architectures enable the first Transformer-based SSL backbone for dense visual prediction tasks.

\vspace{-1mm}
\section{Methods}
\vspace{-3mm}

Transformer-based SSL methods emerge very recently to lead the state-of-the-art performance on the ImageNet linear probe task~\citep{chen2021empirical,caron2021emerging}. It inherits the successes from (1) monolithic Transformer architectures that dominate in NLP~\citep{devlin2019bert,radford2018improving}, and (2) instance-level contrastive learning objectives that demonstrate arguably the best SSL performance in computer vision~\citep{chen2020simple}.
Though simple and effective, the existing Transformer-based SSL methods require a large amount of compute resources (\eg $>$1.7 TPU years of training) to reach SoTA performance.
We believe that the SSL system {\em efficiency} is highly related to two ingredients: the network architecture and the pre-train task. To strike for a better tradeoff between accuracy and efficiency, we present \shortname{}, showing better synergy of networks (a multi-stage Transformer architecture) and pre-train tasks (a non-contrastive region-matching task).

% As common practice, different crops of each image are taken under random data augmentation. Each augmented view is partitioned into non-overlapped patches with patch size $P\!\times\!P$. Concatenating a $\texttt{[CLS]}$ token (as a global token) with these patches,  they are encoded by a stack of Transformer layers with the same network configurations, such as ViT~\citep{dosovitskiy2020image} or DeiT~\citep{touvron2020training}. Hence, the input sequence and output representation share the same number of tokens, and it is clear that each local patch has its unique corresponding top-layer feature representation. The global representation of different views are further projected into a latent space using a shared MLP head, where the similarity among augmented views from the same image is maximized.

% \JG{the last sentence is not clear. Do you mean that the ``the similarities among matched views are maximized''? need to clarify that matched vs. unmatched views. e.g., a view and all its augmented views form a set of matched views.}



\subsection{Network Architectures: From Monolithic to Multi-stage ViT Backbone}
\vspace{-2mm}
% \JG{need to clarify the following points in this section.
% (1) What is the main Challenge of using transformer for vision? It is computationally expensive to perform self-attention for high-resolution images. Given a fixed patch size, the number of tokens grows with the resolution of an image. $O(T^2)$
% (2) The common solution is to multi-stage ViTs, where  at the lower layers, only local patch dependencies are captured in fine-grained, and at the higher layers,  global dependencies are captured in coarse-grained. Therefore, existing ViTs fail to capture global fine-grained dependencies among patches. 
% (3) To address the issue, there have been recent works that introduce new ViT architectures, including ViL, Swin, CvT….
% (4) In this study, instead of proposing a new ViT architecture, we show the issue can be addressed more effectively by incorporating a new pre-training task of region matching.}

\paragraph{Multi-stage ViT.} This paper presents the first empirical study of multi-stage Transformer architectures~\citep{vaswani2021scaling,wang2021pyramid,liu2021Swin,zhang2021vil,wu2021cvt} for SSL. Each stage consists of a {\em patch merging/embedding} module, and a {\em Transformer with sparse self-attention} module.
$(\RN{1})$ The patch merging module plays a slightly different roles in different stages. In the first stage, it splits an input RGB image into non-overlapping
patches. Each patch is treated as a ``token'', constructed as a concatenation of the raw pixel RGB values, which is further projected into a $C$-dimension feature.
In the later stage, the patch merging module concatenates the features of each group of $2\times2$ neighboring patches, and applies a linear layer on the 4$C$-dimensional concatenated features. This reduces the number of tokens by a multiple of $2\times2=4$, and the output dimension is set to $2C$.
$(\RN{2})$ A Transformer with sparse self-attention module are then employed to enable interactions among the merged features. 
The two modules above are repeated for multiple times, typically 4 times, resulting in a multi-stage ViT. As a result, a hierarchical representation is generated: the number of tokens is reduced and the feature dimension (and the number of heads in self-attentions) of each token is increased, as the network
gets deeper. 
An overview comparison of the monolithic and multi-stage Transformer architectures for SSL is illustrated in Figure~\ref{fig:illustration_esvit} in Appendix. 
% We consider three multi-stage ViT in this paper: {\em Swin Transformer}~\citep{liu2021Swin}, {\em Vision Longformer (ViL)}~\citep{zhang2021vil} and {\em  Convolution vision Transformer (CvT)}~\citep{wu2021cvt}, and briefly describe how to adapt the network specifications in our SSL settin in Appendix. 
% Please see Figure~\ref{fig:illustration_esvit} (b) for a brief illustration of this concept.

\paragraph{An intriguing property of self-supervised monolithic ViT.} 
Though straightforward in implementation, changing from monolithic to multi-stage architecture without careful treatments may lose some desirable properties of self-supervised Transformers, as discussed in the following.
In out study, we first empirically note an intriguing property of self-supervised monolithic ViT\citep{caron2021emerging}: {\em the pre-trained model exhibits a very strong ability to automatically discovers correspondences, even without a region-level matching objective specified in training}. To illustrate this property, in Section \ref{sec:correspondence_imagenet} in Appendix, we quantitatively show that a self-supervised monolithic ViT yields {\bf 95\%} accuracy in successfully identifying the correct region-to-region correspondences for 50K images on the ImageNet validation dataset. However, simply replacing the network with a multi-stage Transformer yields only {\bf 66\%} accuracy. This significant degradation (absolute {\bf 29\%} accuracy drop) reveals the loss of the correspondence learning property. We first raise this critical problem, and believe that it has a large impact on the pre-trained model's performance in various downstream tasks.

% In computing self-attention, we follow  by including a relative position bias $B \in \R^{M2xM2}$ to each head in computing similarity: Since the relative position along each axis lies in the range $[-M+1, M-1]$, we parameterize a smaller-sized bias matrix $\hat{B} \in \R^{(2M-1) \times (2M-1)}$, and values in B are taken from $\hat{\Bmat}$.

\vspace{-2mm}
\subsection{Pre-training Tasks: Delving into Views with Regions}
\vspace{-2mm}
We employ a non-contrastive learning framework to build our SSL method. Specifically, {\em Self-distillation with no labels} (DINO)~\citep{caron2021emerging} is considered. It leverages the knowledge distillation learning paradigm where a student network $g_{\thetav_s}$ is trained
to match the output of a given teacher network $g_{\thetav_t}$
, parameterized by $\thetav_s$ and $\thetav_t$ respectively. 
The neural network $g$ is composed of a backbone $f$ (\eg Transformers or ConvNets), and of a projection head $h$: $g = h \circ f$. The features used in downstream tasks are the output of backbone $f$.
%
In SSL, different augmented views $\Tilde{\xv}$ of an image $\xv$ are fed into backbone network to obtain feature maps $\zv =f(\Tilde{\xv})$. Two MLP heads followed by \texttt{softmax} per network further convert the feature vectors $z \in \zv$ into probability vectors $p=h(z)$; one head for view-level and the other head for region-level, respectively.  

More precisely, from a given image, we generate a set $\Vcal$ of different views\footnote{This set often contains views of two different resolutions $\Vcal = [\Vcal_g, \Vcal_l  ]$, where $\Vcal_g = \{ \Tilde{\xv}_{g_i} | i=1,2 \}$ is a global-view set of higher resolution, and $\Vcal_l = \{ \Tilde{\xv}_{l_i} | i=1,\dots,8 \}$  is a local-view set of lower resolution. All views $\Vcal$  are passed through the student while only the global views $\Vcal_g$ are passed through the teacher.} following~\citep{caron2021emerging}. 
%
The resulting feature map at the top layer for each view is $\zv = [z_1, \dots, z_T] $, where $T$ is the sequence length, and $z_i$ is a region-level representation for the local patch at position $i$. Average pooling is applied to obtain the view-level representation $\bar{z}= \text{avg-pool} (\zv)$.  


\paragraph{View-level task}
Given the augmented view set for student $ \Vcal$ and teacher $ \Vcal^*$, a set of pairs $ \Pcal = \{ (s,t) | \Tilde{\xv}_s \in \Vcal,  \Tilde{\xv}_t \in \Vcal^*  \text{~and~} s \neq t $ \} is constructed to perform cross-view prediction tasks. We consider the pre-training task at the view level proposed by~\citep{caron2021emerging}:
%
\begin{align}\label{eq:obj_view}
\Lcal_V = \frac{1}{| \Pcal|} \sum_{ (s, t) \in \Pcal }  
\Mcal_V ( s, t), ~~\text{with} ~~
 \Mcal_V (s, t ) = -  p_{s} \log p_t,
\end{align}
%
where 
$p_s = h(\bar{z}_s)$ and $p_t = h(\bar{z}_t)$ are the probability output of an MLP head $h$ over the view-level representations $\bar{z}_s$ and $\bar{z}_t$, learned by student and teacher, respectively. In DINO, ViT/DeiT are considered, hence the view-level representation is the feature of the $\texttt{[CLS]}$ token.

\paragraph{Region-level task}
In~\citep{caron2021emerging}, the $\Lcal_{V}$ encourages ``local-to-global'' correspondences only at a coarse level: the large crop and the small crop are matched in the view level, leaving region-to-region correspondence unspecified. In monolithic Transformers, the drop paths and skip connections from low-level features to high-level features help the the latter to remain discriminative, thus maintain good region-matching performance. However, such a property gets diluted due to the merging operators in multi-stage Transformers. As shown in our experiments later, training a multi-stage network with $\Lcal_{V}$ only indeed results in sub-optimal representations, though network efficiency is greatly improved.

Further, it could be a waste of computation not to leverage region-level features $\zv$ that are computed in the process of extracting view-level feature.
Inspired by the success of masked language modeling task in BERT, we argue that it is important to have region-level pre-training task for computer vision, so that the model can (1) amortize the computation and fully leverage the extracted region-level features, and (2) take into account the co-occurrences/structures between local features. Unfortunately, directly performing masked patch
prediction (MPP) for the multi-stage Transformer architecture is infeasible, as the one-to-one correspondences between the input visual tokens and output features get diluted due to the merging operation. Even for monolithic architectures, MPP has not been proved effective in computer vision, as empirically shown in~\citep{dosovitskiy2020image}.

\label{sec:correspondence_imagenet}


To address this problem, we propose a non-contrastive, region-matching method
that directly works at the level of local features
by taking into account their correspondences:
%
\begin{align}\label{eq:obj_region}
\vspace{-2mm}
\hspace{-2mm}
 \Lcal_R = \frac{1}{| \Pcal|}  \sum_{ (s, t) \in \Pcal }  
\Mcal_R ( s, t), ~~\text{with} ~~
 \Mcal_R (s, t ) = - \frac{1}{T}\sum_{i=1}^T  p_{j^*} \log p_i, ~~ j^* = \arg \max_{j} \frac{z_i^T z_j}{\|z_i\| \|z_j\|},
\end{align}
where 
$p_i = h^{\prime}(z_i)$ and $p_j = h^{\prime}(z_j)$ are the probability outputs of a new MLP head $h^{\prime}$ over the local features of student $z_i \in \zv_s$ and teacher $z_j \in \zv_t$, respectively. $j^*$ is the index of the feature in $\zv_t$ that best matches the $i$-th feature in $\zv_s$, in the sense of highest cosine similarity. 

%
\begin{wrapfigure}{R}{0.5\textwidth}
\vspace{-5mm}
\begin{minipage}{0.5\textwidth}
\scriptsize
\centering
\hspace{-3mm}
\includegraphics[height=3.2cm]{figs/esvit_preidctions.pdf}
\vspace{-1mm}
\caption{Pre-training objectives, including view-level  (left) and region-level (right) prediction.} 
\label{fig:esvit_preidctions}
\vspace{-3mm}
\end{minipage}
\end{wrapfigure}
%
The overall pre-training objective of \shortname{} is $\Lcal = \Lcal_R + \Lcal_V$, we learn to match the feature distributions at both the view and region levels by minimizing the cross-entropy loss w.r.t. the parameters of the student network $g_{\thetav_s}$. A visual illustration is in Figure~\ref{fig:esvit_preidctions}, and the full algorithm is in Appendix. 
We updates teacher/student network alternatively:
%
$(\RN{1})$ Given a fixed teacher network, the student network is updated by minimizing the full cross-entropy loss:
$\thetav_s  \leftarrow \arg \min_{\thetav_s} \Lcal(s, t ; \thetav_s)$.
$(\RN{2})$ The teacher model is updated as an exponential moving average (EMA) of the student weights
$\thetav_t  \leftarrow \lambda \thetav_t + (1 - \lambda) \thetav_s$, with $\lambda$  following a cosine schedule
from 0.996 to 1 during training.
%
By default, the full objective $\Lcal$ is used from the beginning. One can also load a checkpoint trained by $\Lcal_V$ only, and add $\Lcal_R$ for continual pre-training, which is shown effective in boosting performance in our experiments.

\paragraph{Computational overhead}
Note that applying $\Lcal_R$ on the traditional monolithic Transformer architecture can be prohibitively computationally expensive, as it requires $\Ocal(T^2)$ to compute $\Lcal_R$. For a typical image of resolution $224 \!\times \!224$, the feature map length  of ViT/DeiT (with patch size 16) at the top layer is $T=196$, while the multi-stage architecture yields $T=49$, which requires 3 times less compute in computing $\Lcal_R$. To empirically illustrate this, we show in Appendix Section~\ref{sec:lr_efficiency} that $\Lcal_R$ adds acceptable extra memory and computational cost (around 1.2 and 1.05 $\times$, respectively) for multi-stage Transformers, while it will quickly go out-of-memory for monolithic Transformers when the batch size is increased.


% \subsection{Discussion of Related Region-level Tasks}
\vspace{-3mm}
\section{Related Works}
\vspace{-3mm}

\paragraph{Relation to mask prediction tasks} We can consider the proposed $\Lcal_R$ as a proxy to mimick masked language modeling in BERT, where the ``ground-truth'' local token is a soft label provided by the teacher network, while the student network makes predictions to match that target, based on the context of regions in a different augmented view. Importantly, our $\Lcal_R$ considers \texttt{softmax} with cross-entropy in the objective, rather than \texttt{MSE} as in MPP. A very sharp teacher distribution is used by choosing small temperatures. This encourages the model to focus on the salient dimensions, rather than waste modeling capability on training short-range dependencies and high-frequency details~\citep{ramesh2021zero}.

\paragraph{Relation to DenseCL} The proposed $\Lcal_R$ mostly related to DenseCL~\citep{wang2020dense} in that the region correspondences in both methods are determined as the two most similar grid features. One critical difference is that DenseCL is a contrastive region-matching task, while our $\Lcal_R$ is a non-contrastive region-matching task, where no negative samples/queue is needed. This technical difference has a significant impact on the downstream task performance. We find that $\Lcal_R$ is particularly effective in serving our goal to improve image classification performance and build efficient \& affordable SoTA SSL system; In contrast, DenseCL degrades the classification performance. 

\paragraph{Relation to other region-level tasks} The ideas of leveraging local region-level pre-training tasks for visual representation learning have been explored for ConvNets~\citep{misra2020self,xiong2020loco,wang2020dense,xie2021detco,yang2021instance,xie2021propagate}. We summarize the differences in three aspects:
$(\RN{1})$
Motivation. Our region-matching task $\Lcal_R$ aims to recover the lost property of automatic correspondence learning in self-supervised monolithic Transformers, while most existing region-level tasks aim to improve dense visual prediction tasks.
$(\RN{2})$ 
Technical difference. Our $\Lcal_R$ is a non-contrastive region-matching task, while others are contrastive learning.
$(\RN{3})$
Empirical performance. Most region-level tasks improve dense visual prediction tasks but sacrifice their image classification performance, while $\Lcal_R$ consistently improves classification performance. Among them, \shortname{} training method achieves the best ImageNet linear probe performance with minimum computational overhead. For detailed comparisons, please refer to Table~\ref{table:region_level_tasks} in Appendix.


\paragraph{Self-supervised vision Transformers.} The research on Transformer-based self-supervised representation learning just scratches the tip of the iceberg, and only a few attempts are made on this topic.  ImageGPT~\citep{chen2020generative} and MoCo-v3~\citep{chen2021empirical} dedicate huge compute resource with large models to exploring the frontier. 
DINO~\citep{caron2021emerging} achieves comparable performance of large self-supervised ConvNets using small/medium-size Transformers. The proposed \shortname{} further pursues efficient and affordable solutions to self-supervised vision Transformers.
%
For more general related works on Transformers for vision tasks and self-supervised ConvNets, please refer to Section~\ref{sec:related_work_appendix} in Appendix. 

% DeiT~\citep{touvron2020training}, 
% Swin Transformer~\citep{liu2021Swin}, 
% Vision Longformer (ViL)~\citep{zhang2021vil}, 
% Convolutions vision Transformers (CvT)~\citep{wu2021cvt}, 
% Pyramid vision Transformer (PvT)~\citep{wang2021pyramid}
% ViT~\citep{dosovitskiy2020image}


% Note that footnotes are properly typeset \emph{after} punctuation marks.\footnote{As in this example.}



\vspace{-3mm}
\section{Experimental Results}
\vspace{-3mm}
%
We describe the experimental settings in Appendix Section~\ref{sec:experimental_settings}, and evaluate the proposed \shortname{}{} to answer three questions:
\textbf{\texttt{Q1}}: How does \shortname{} perform on standard ImageNet benchmark compared to SoTA methods?
\textbf{\texttt{Q2}}: How effective \shortname{} is when transferring to downstream tasks? 
\textbf{\texttt{Q3}}: What are the design choices and empirical contributions of $\Lcal_R$? 
\textbf{\texttt{Q4}}: When does the intriguing property of self-supervised Transformers exist, including learned correspondence and attentions?


\begin{table}[t!]
\footnotesize % \small
\centering
\scalebox{0.89}{
\begin{tabular}{ @{\hspace{-0pt}}l@{\hspace{8pt}}c@{\hspace{2pt}}@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c}%rrrrrrrrrrrr
\toprule
 Method   &  \#Parameters $\downarrow$~~ &  Throughput (Image/s) $\uparrow$ & Linear $\uparrow$~~ & $k$-NN $\uparrow$  \\ 
\hline
\multicolumn{3}{l}{\em \hspace{-3mm} SoTA SSL methods with Big ConvNets}  & & \\
SwAV, RN50w5~\citep{caron2020unsupervised} & 586 & 76 & 78.5 &  67.1 \\
BYOL, RN200w2~\citep{grill2020bootstrap} & 250 & 123 & 79.6 & 73.9 \\
SimCLR-v2, RN152w3+SK ~\citep{chen2020big} & 794 & 46 & 79.8 & 73.1 \\
\midrule
\multicolumn{5}{l}{\em \hspace{-3mm} Skyline methods with excessively long sequences for self-attentions}  \\
DINO, DeiT-S/8~\citep{caron2021emerging} & 21 & 180 & 79.7 & 78.3 \\
DINO, ViT-B/8~\citep{caron2021emerging} & 85 & 63 & 80.1 & 77.4 \\
MoCo-v3, ViT-B-BN/7~\citep{chen2021empirical} & 85 & $\sim$63 & 79.5 & - \\
MoCo-v3, ViT-L-BN/7~\citep{chen2021empirical} & 304 & $\sim$17 & 81.0 & - \\
iGPT, iGPT-XL~\citep{chen2020generative} &  6801 & - & 72.0 & - \\
\rowcolor{Gray}
\shortname{}, Swin-S/$W\!=\!14$ & 49 & 383   &  80.8   &   79.1 \\
\rowcolor{Gray}
\shortname{}, Swin-B/$W\!=\!14$ & 87 & 254   &  {\bf 81.3}   &  {\bf 79.3} \\
\midrule
\multicolumn{5}{l}{\em \hspace{-3mm} Transformer-based SSL, with moderate sequence length for self-attentions}  \\
\textcolor{gray}{Masked Patch Pred., ViT-B/16~\citep{dosovitskiy2020image}} & \textcolor{gray}{85} & \textcolor{gray}{312} &  ~\textcolor{gray}{79.9}$^{\dagger}$ & - \\
DINO, DeiT-S/16~\citep{caron2021emerging} & 21 & 1007 & 77.0 & 74.5 \\
DINO, ViT-B/16~\citep{caron2021emerging} & 85 & 312 & 78.2 & 76.1 \\
MoCo-v3, ViT-B/16~\citep{chen2021empirical} &  85  & 312 & 76.7 & - \\
MoCo-v3, ViT-H-BN/16~\citep{chen2021empirical} & 632 & $\sim$32 & 79.1 & - \\
MoBY, Swin-T~\citep{xie2021moby} & 28 &  808 & 75.1 & - \\
\rowcolor{Gray}
\shortname{}, Swin-T & 28 &  808 &  78.1  & 75.7 \\
\rowcolor{Gray}
\shortname{}, Swin-S & 49 &  467 &  79.5  & 77.7 \\
\rowcolor{Gray}
\shortname{}, Swin-B & 87 &  297 &  {\bf 80.4}  & {\bf 78.9} \\
\bottomrule
\end{tabular} }

% \rowfont{\color{gray}}

\vspace{0mm}
\caption{Comparison with SoTA across different architectures on ImageNet linear probing. ViT-BN is ViT that has BatchNorm~\citep{frankle2020training}, and “$/P$” denotes a patch size of $P\!\times\!P$. ``$\sim$'' indicates through-puts estimated by comparing different papers, detailed in Appendix. $^{\dagger}$ The mask patch prediction in~\citep{dosovitskiy2020image} is pre-trained on JFT-300M and end-to-end fine-tuned in ImageNet, which we append as a reference.}
\label{tab:main_result_cls}
\vspace{-5mm}
\end{table}




% \begin{table}[t!]
% \footnotesize % \small
% \centering

% \begin{tabular}{ @{\hspace{-0pt}}l@{\hspace{8pt}}|c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c}%rrrrrrrrrrrr
% \toprule
%  Arch.   &  Objectives & Window & Linear & $k$-NN  \\ 

% \hline
% \multirow{3}{*}{Swin-Tiny}
% & $f_{V}$ & 7 & 77.0 & 74.2 \\
% & $f_{V}$ & 14 & 77.9 & 75.5 \\
% & $f_{V}+f_{R}$ & 7 &  78.1  &  75.7 \\
% & $f_{V}+f_{R}$ & 14 &  {\bf 78.7}  & {\bf 77.0} \\
% \midrule
% \multirow{3}{*}{Swin-Small}
% & $f_{V}$ &  7 & 79.2  & 76.8  \\
% & $f_{V}$  & 14 &   &    \\
% & $f_{V}+f_{R}$ & 7 &  {\bf 79.5}  & {\bf 77.7}  \\
% & $f_{V}+f_{R}$ & 14 &     &    \\
% \bottomrule
% \end{tabular} \\

% \vspace{2mm}
% \caption{Ablations of pre-training tasks and window sizes.}
% \label{tab:cmp_obj}
% \vspace{-0mm}
% \end{table}


% \begin{figure*}[h!]%\vspace{-25pt}
% \vspace{-0mm}\centering 
% \centering
% \hspace{-3mm}
% \includegraphics[height=3.9cm]{figs/obj_view_and_region.pdf}
% \vspace{-1mm}
% \caption{Learning curves of different objectives.} 
% \label{fig:obj_curves}
% \vspace{-3mm}
% \end{figure*}

\vspace{-3mm}
\subsection{Comparisons with Prior Art on ImageNet}
\label{sec:imagenet_probe}
\vspace{-3mm}
We report top-1 linear probe and $k$-NN classification accuracy  on the ImageNet validation set.
%
Table~\ref{tab:main_result_cls} presents comparisons with all SoTA SSL vision systems across various network architectures. Please refer to Figure~\ref{fig:hero_cmp} for visual comparisons over scaling parameter counts and throughput. Our main findings are summarized below.

\paragraph{Comparisons with self-supervised Transformers.} 

% Both iGPT~\citep{chen2020generative} and the masked patch prediction in~\citep{dosovitskiy2020image} are earlier variants of masked auto-encoding schemes, mimicking the behaviors of GPT~\citep{radford2018improving} and BERT~\citep{devlin2019bert} in NLP, respectively. 

The DINO- and MoCo-based ViT has higher accuracy and smaller models than iGPT, under the same linear probing protocol and training data. At the similar level of model size and compute complexity, the proposed \shortname{} improve SoTA methods DINO/MoCo-v3 by a large margin: \shortname{} (Swin-B) outperforms  DINO (ViT-B/16) by 2.2\% linear probe accuracy and 2.8\% $k$-NN accuracy in absolute values.
\shortname{} (Swin-B) even performs slightly better than DINO (ViT-B/8) (0.3\% higher linear probe accuracy and 1.5\% higher $k$-NN accuracy), with $4\times$ higher throughput.
MoBY~\citep{xie2021moby} is a con-current work that investigates multi-stage ViT in SSL. With the same architecture Swin-T, our \shortname{} pre-training tasks significantly outperform MoBY, showing 3\% higher accuracy. 
In \shortname{}, longer sequences in self-attention is implemented by increasing the window size. We experiment this by considering a window size of $W\!=\!14$. 
Overall, the proposed \shortname{} (Swin-B/$W$=14) shows the best performance (top-1 accuracy 81.3\%, top-5 accuracy 95.5\%, $k$-NN accuracy 79.3\%), compared with all systems, and is $3.5\times$ parameter-efficient and has at least $10\times$ higher throughput than previous SoTA MoCo-v3. 


% Our smaller model  \shortname{} (Swin-S/$W$=14) achieves 80.8\% top-1 accuracy, approaching SoTA (81.0\%, MoCo-v3 with ViT-BN-L/7~\citep{chen2021empirical}) with  $6\times$ less parameters and $22\times$ higher throughput, and outperforms the 2nd place method (80.1\%, DINO with ViT-B/6~\citep{caron2021emerging}), with $1.5\times$  less parameters and $6\times$ higher throughput. We leave the study of further scaling \shortname{} as future work.

% \CL{ToDO, where to put?} Our self-supervised model \shortname{} has larger improvement gaps when the models are bigger than the supervised results in~\citep{liu2021Swin}. For example, from Swin-S to Swin-B, \shortname{} shows an accuracy improvement of 0.9\%, while supervised learning shows 0.3\%  improvement when trained in ImageNet-1K.



\paragraph{Comparisons with big ConvNets.}
We compare with the SoTA big ResNets reported by SimCLR-v2~\citep{chen2020big}, BYOL~\citep{grill2020bootstrap} and SwAV~\citep{caron2020unsupervised}. Among them, the best accuracy $79.8\%$ under the linear probing protocol is reported by SimCLR-v2 with SK-ResNet, where Selective Kernel (SK)~\citep{li2019selective} is a form of attention to enhance CNNs. 
It is clear in Figure~\ref{fig:hero_cmp} (b) that all ConvNets-based SSL methods show an envelope in the regime of scaling up model sizes after passing $500$M.
\shortname{} achieves better accuracy than their highest envelope, with $16\times$ less model parameters and $8\times$ higher throughput.

% \paragraph{Longer sequences for self-attentions.} It is observed that using longer sequences in self-attentions can improve recognition accuracy: In iGPT~\citep{chen2020generative} sequence length is increased in the pixel domain; DINO and MoCo-v3 explore longer sequences by reducing the patch size to $8\times8$ or $7\times7$ (``/8'' or``/7'' in Figure~\ref{fig:hero_cmp} and Table~\ref{tab:main_result_cls}), respectively. This keeps the model parameter counts unchanged, but dramatically increases compute complexity (measured by increased FLOPs and decreased throughput), \eg to around $6\times$ reported in MoCo-v3. 
% This reveals that small patches provide gains.
% In \shortname{}, longer sequences in self-attention is implemented by increasing the window size. We experiment this by considering a window size of $W\!=\!14$, and report the results in Table~\ref{tab:cmp_obj}, where we see a consistent accuracy improvement of around 1-2\%. In Table~\ref{tab:main_result_cls}, \shortname{} with Swin-S/$W\!=\!14$  achieves highest 79.1\% $k$-NN accuracy, and comparable linear probe accuracy with SoTA, with almost an order of magnitude higher efficiency.  





\vspace{-2mm}
\subsection{Transfer Learning}
\vspace{-2mm}
We also conduct transfer learning in downstream tasks to evaluate the quality of learned representations. Two sets of tasks are considered:


\begin{minipage}{0.99\textwidth}
\centering

\begin{itemize}[leftmargin=5.5mm]
\item {\em Classification on a suite of 18 small datasets}. As exemplified in \citep{radford2021learning}, it is a common and clean approach to evaluate a learned representation by fitting a linear classifier on
the representation and measuring its performance across multiple datasets.  We study 18 datasets used in~\citep{radford2021learning}. Automatic hyper-parameter tuning is considered to ensure fairness of comparison. Besides averaged $\texttt{scores}$, we report $\texttt{\#\!\! wins}$ as the number of datasets on which the model outperforms its supervised counterpart. Detailed dataset description and settings are in Appendix.
\end{itemize}

\end{minipage}

\begin{minipage}{0.99\textwidth}
\centering

\begin{itemize}[leftmargin=5.5mm]
\item {\em Detection and segmentation on COCO}. Different from previous monolithic self-supervised ViT, the multi-stage architecture in \shortname{} can be readily used for dense visual tasks that require hierarchical feature representations.
\end{itemize}
\vspace{-2mm}
\end{minipage}


\paragraph{Comparison with supervised counterparts.} We compare with the supervised-learning Swin, whose checkpoints are downloaded from the official codebase\footnote{\url{https://github.com/microsoft/Swin-Transformer}}. 
Figure~\ref{fig:esvit_transfer_cls} shows the classification results of Swin-S, \shortname{} consistently outperforms its supervised variant, often by a large margin. Similar conclusions are drawn for other model sizes. On COCO detection and segmentation task, however, comparable results with the supervised counterpart are obtained, as shown in Table~\ref{table:coco_res} for Swin-T. We hypothsize this is related to the non-constrastive nature of \shortname{}, as explained later.



\begin{figure*}[t!]%\vspace{-25pt}
\vspace{-0mm}\centering 
\centering
\hspace{-3mm}
\includegraphics[height=3.9cm]{figs/transfer_cls_swin_small.pdf}
\vspace{-2mm}
\caption{Transfer learning to a wide variety of datasets. Fitting a linear
classifier on \shortname{}’s features outperforms using its supervised  counterpart on 17 out of 18 datasets.} 
\label{fig:esvit_transfer_cls}
\vspace{-2mm}
\end{figure*}





\begin{table}[t!]
\begin{minipage}[b]{0.43\linewidth}

  \centering
  \scalebox{0.92}{
  \begin{tabu}{l |  lll }
    \toprule
   & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$   \\ \cline{2-4}
   % \midrule
    \rowfont{\color{gray}}
    Supervised &  46.0 & 68.1 & 50.3   \\
    \shortname{}  & 46.2 & 68.0 & 50.6   \\
    \midrule
   &  AP$^{mb}$ & AP$^{mb}_{50}$ & AP$^{mb}_{75}$  \\ \cline{2-4}
    % \midrule
    \rowfont{\color{gray}}
    Supervised & 41.6 & 65.1 & 44.9  \\
    \shortname{} & 41.6 & 64.9 & 44.8  \\
    \bottomrule
  \end{tabu}
  }
  \vspace{-2mm}
  \caption{COCO Detection \& Segmentation.}
  \vspace{-2mm}
  \label{table:coco_res}  
\end{minipage}\hfill
\begin{minipage}[b]{0.57\linewidth}
  \centering
  \scalebox{0.83}{
  \begin{tabu}{l | cc | cc}
    \toprule
    Pre-train Data    
    &   \multicolumn{2}{c|}{ImageNet-1K}  
    & \multicolumn{2}{c}{18 Datasets}    \\
          &   Linear & $k$-NN & Scores & \# Wins \\
    \midrule
    \rowfont{\color{gray}}
    Supervised & - & -  &  77.29 & - \\
    ImageNet-1K &  78.0 {\footnotesize (77.1)}  & 75.7 {\footnotesize (73.7)}  & 80.66  & 16 \\
    WebVision-v1    & 75.9 {\footnotesize (75.4)} &  71.2 {\footnotesize (69.4)} & 80.00 & 14 \\ 
    OpenImages-v4    & 70.6 {\footnotesize(69.6)} &  62.0 {\footnotesize (60.3)}   & 77.97 & 10 \\
    ImageNet-22K   & 75.0 {\footnotesize(73.5)} & 67.9 {\footnotesize (66.1)}  & {\bf 81.03} & {\bf 17} \\    
    \bottomrule
  \end{tabu}
  }
  \vspace{-2mm}
  \caption{Impact of the pre-train datasets.}
  \vspace{-2mm}
  \label{table:datasets_res}  
\end{minipage}
  \vspace{-8mm}
\end{table}

\paragraph{Effects of larger, less-curated pre-train datasets.}
The performance of Transformer-based SSL research has thus far been limited to highly curated pre-train data such as ImageNet-1K. To push the frontier in leveraging large amounts of unlabeled data, we explore the effects of pre-training from larger, less-curated image datasets:  
WebVision-v1~\citep{li2017webvision}, OpenImages-v4~\citep{kuznetsova2020open} and ImageNet-22K~\citep{deng2009imagenet}, described in Appendix. The pre-train epochs on different datasets are adjusted so that all models see a similar number of augmented views. 
We summarize the results in Table~\ref{table:datasets_res} and would like to emphasize the following findings.
First, $\Lcal_R$ improves $\Lcal_V$ (shown in parentheses) on all datasets.
Second, all \shortname{} pre-trained checkpoints outperform supervised checkpoint in downstream classification tasks, but performance varies a lot, with ImageNet-22K checkpoint showing the best transfer ability. Third, ImageNet-1K pre-trained model shows the best ImageNet-1K linear probe performance. 
We hypothesize that it is not only the size of pre-train dataset matters, but also the distribution of image classes matters: more diverse and well-balanced distribution results in a stronger generalization ability. 
% Similar observations are reported in a concurrent work~\citep{tian2021dnc} for ConvNets.





% \begin{table}
%   \centering
%   \scalebox{0.80}{
%   \begin{tabu}{l | cc | llllll| cc}
%     \toprule
%     Pre-train     
%     &   \multicolumn{2}{c|}{ImageNet-1K}  
%     &  \multicolumn{6}{c|}{  COCO Detection  \& Segmentation} & \multicolumn{2}{c}{Classification on 18 Datasets}    \\
%           &   Linear & $k$-NN  & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$  &  AP$^{mb}$ & AP$^{mb}_{50}$ & AP$^{mb}_{75}$  & Scores & \# Wins \\
%     \midrule
%     \rowfont{\color{gray}}
%     Supervised & - & - &  46.0 & 68.1 & 50.3  & 41.6 & 65.1 & 44.9   &  77.29 & - \\
%     ImageNet-1K &  77.1 & 73.7  & 46.2 & 68.0 & 50.6 & 41.6 & 64.9 & 44.8 & 80.66  & 16 \\
%     WebVision-v1    & 75.4 &  69.4 &   &  &  &   & & & 80.00 & 14 \\ 
%     OpenImages-v4    & 69.6 &  60.3  & 46.0 &  67.6 & 50.6 & 41.3 & 64.5 & 44.1 & 77.97 & 10 \\
%     ImageNet-22K   & 73.1 & 66.1 & 46.0 & 67.9 & 50.8  &  41.6 & 64.9 & 44.7  & {\bf 81.03} & {\bf 17} \\    
%     \bottomrule
%   \end{tabu}
%   }
%   \vspace{2mm}
%   \caption{Impact of the pre-training datasets for \shortname{} in transfer learning.  The supervised Swin-T checkpoint is downloaded from the official codebase.}
%   \label{table:coco}  
% \end{table}


\vspace{-2mm}
\subsection{Discussion on the Non-contrastive Region-Matching Task}
\vspace{-2mm}


\begin{wraptable}{r}{7.3cm}
% \begin{table}[t!]
\footnotesize % \small
\centering
\vspace{-5mm}
\scalebox{0.80}{
\begin{tabular}{ @{\hspace{8pt}}c@{\hspace{2pt}}@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}|c@{\hspace{8pt}}|c@{\hspace{8pt}}c@{\hspace{8pt}}}%rrrrrrrrrrrr
\toprule
\multirow{1}{*}{Method}    &  \multirow{1}{*}{\#Param.}  &   \multirow{1}{*}{ Im./s} &  Pre-train tasks   &   Linear & $k$-NN  \\
%   &  &  & pre-train tasks & Linear & $k$-NN \\ 
\midrule
DeiT & 21 &  1007 & $\Lcal_{V} $  & 75.9  &  73.2 \\ \midrule
\multirow{3}{*}{R-50} & \multirow{3}{*}{24} &  \multirow{3}{*}{1237}   &  $\Lcal_{V}$  &  ~75.3$^{\dagger}$ & ~67.5$^{\dagger}$ \\
 &  &   &   $\Lcal_{V}$  & 75.0 &  69.3 \\ 
 &  &   &   $\Lcal_{V}\!+\!\Lcal_{R}$    & {\bf 75.7}  &  {\bf 71.2} \\ \midrule
\multirow{2}{*}{Swin} & \multirow{2}{*}{28} &  \multirow{2}{*}{808}   &  $\Lcal_{V} $  & 77.1 &  73.7 \\
 &  &   &   $\Lcal_{V}\!+\!\Lcal_{R}$    & {\bf 77.6}  &  {\bf 75.4} \\ \midrule
\multirow{2}{*}{ViL} & \multirow{2}{*}{28} &  \multirow{2}{*}{386}     &  $\Lcal_{V} $  & 77.3 &  73.9 \\
 &  &    &   $\Lcal_{V}\!+\!\Lcal_{R}$    & {\bf 77.5}  &  {\bf 74.5}  \\ \midrule
\multirow{2}{*}{CvT} & \multirow{2}{*}{29} &  \multirow{2}{*}{848}  
 &   $\Lcal_{V} $  & 77.6  & 74.8  \\
 &  &    &  $\Lcal_{V}\!+\!\Lcal_{R}$   &  {\bf 78.5}   & {\bf 76.7}  \\ \midrule
\multirow{2}{*}{PvT} & \multirow{2}{*}{24} &  \multirow{2}{*}{851}  
 &   $\Lcal_{V} $  & 75.4  &  72.0 \\
 &  &    &  $\Lcal_{V}\!+\!\Lcal_{R}$   &  {\bf 76.3}   & {\bf 72.9}  \\
 
 
 
% \midrule
% \multirow{4}{*}{300}
%  & DeiT & 21 &  1007 & 75.9  &  73.2 \\ \cline{2-6}
%  & Swin & 28 &  808 & 77.1 &  73.7 \\
%  & ViL & 28 &  386 & 77.3 &  73.9 \\
%  & CvT & 29 &  848 & 77.6  & 74.8  \\
\bottomrule
\end{tabular}} \\
%
\vspace{-1mm}
\caption{Different architectures with and without $\Lcal_{R}$. DeiT and ResNet-50 are shown as references. $^{\dagger}$ indicates numbers reported in~\citep{caron2021emerging}. }
\label{tab:cmp_attn_appendix}
\vspace{-2mm}
\end{wraptable}



% \begin{wraptable}{r}{7.9cm}
% % \begin{table}[t!]
% \footnotesize % \small
% \centering
% \vspace{-5mm}
% \begin{tabular}{ @{\hspace{8pt}}c@{\hspace{2pt}}@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}|c@{\hspace{5pt}}c@{\hspace{5pt}}|c@{\hspace{5pt}}c}%rrrrrrrrrrrr
% \toprule
% \multirow{2}{*}{Method}    &  \multirow{2}{*}{\#Param.}  &   \multirow{2}{*}{ Im./s} & \multicolumn{2}{c|}{100 epochs}   &  \multicolumn{2}{c}{300 epochs}  \\ 
%   &  &  & Linear & $k$-NN & Linear & $k$-NN \\ 
% \hline
% DeiT & 21 &  1007 & 73.1  &  69.0 & 75.9  &  73.2 \\ %  \cline{2-6}
% Swin & 28 &  808 & 75.3  &   70.0 & 77.1 &  73.7 \\
% ViL & 28 &  386   &  75.4 & 70.1 & 77.3 &  73.9 \\
% CvT & 29 &  848  &  75.5 &  70.6 & 77.6  & 74.8  \\
% % \midrule
% % \multirow{4}{*}{300}
% %  & DeiT & 21 &  1007 & 75.9  &  73.2 \\ \cline{2-6}
% %  & Swin & 28 &  808 & 77.1 &  73.7 \\
% %  & ViL & 28 &  386 & 77.3 &  73.9 \\
% %  & CvT & 29 &  848 & 77.6  & 74.8  \\
% \bottomrule
% \end{tabular} \\
% %
% \vspace{0mm}
% \caption{Different sparse attentions in \shortname{}.}
% \label{tab:cmp_attn}
% \vspace{-5mm}
% \end{wraptable}



\paragraph{Compatibility with various network architectures.} We investigate ResNet-50 and different efficient sparse Transformers in Table~\ref{tab:cmp_attn_appendix}. DeiT is shown as a baseline reference. Batch size = 1024 in this experiment. To ensure fair comparison, we modify all into a 4-stage architecture with the number of Transformer layers in each stage as 2-2-6-2. We see that $\Lcal_R$ improves all network architectures, including ResNet-50, Swin~\citep{liu2021Swin}, ViL~\citep{zhang2021vil}, CvT~\citep{wu2021cvt} and PvT~\citep{wang2021pyramid}. 
Though directly adding $\Lcal_R$ to monolithic ViT is computationally infeasible, we uniformly sampled top-layer grid features of DeiT and then add $\Lcal_R$, but did not observe performance improvement. This is partly because the monolithic ViT itself already has a good corresponding ability, an extra region-matching task does not provide new learning signals.  As compared in Appendix Table~\ref{table:r50_linear_probe} with the ResNet-50 backbone, \shortname{} learning method shows the highest accuracy, compared with existing SSL methods.

% We choose to scale up Swin in our experiments first to study the limit of \shortname{}, leave the scaling of others as future work.


\paragraph{Model scaling with $\Lcal_R$.} We compare the pre-training objective with and without $\Lcal_R$ in Table~\ref{tab:cmp_obj}. Across different model scales and window sizes, the proposed region level $\Lcal_R$ can consistently improve the performance. The gains can be clearly seen by $k$-NN accuracy (around 1-2\%),  where no additional tuning is needed as in linear probe. Figure~\ref{fig:obj_curves} demonstrates that $\Lcal_R$ helps model convergence, and can be used as a drop-in to improve models trained with the view level task.

\paragraph{Contrastive {\em vs} Non-contrastive region-matching tasks.} The proposed $\Lcal_R$ adds a non-contrastive region-matching task to the non-contrastive view-level task $\Lcal_V$; On the contrary, DenseCL adds a contrastive region-matching task to the contrastive view-level task MoCo-v2. In Table~\ref{table:region_matching}, we compare four methods in the same setting with ResNet-50. DenseCL improves dense visual prediction performance, but hurts classification performance. $\Lcal_R$ improves both tasks, especially the classification performance. One limitation is that the non-contrastive methods show lower performance in dense prediction tasks, this is consistent with the observations for BYOL in~\citep{wang2020dense}.
The simple $\Lcal_R$ shows the best ImageNet accuracy compared with all sophisticated region-level tasks in this 200-epoch setting in Appendix Table~\ref{table:region_level_tasks}, and the best overall accuracy in Table~\ref{table:r50_linear_probe}. It indicates that $\Lcal_R$ well serves our goal in building efficient SoTA SSL systems.

\paragraph{Design choices of $\Lcal_R$.} We ablate a couple of choices in constructing $\Lcal_R$ in Eq. \eqref{eq:obj_region}. 
$(\RN{1})$ \texttt{Softmax} {\em vs} \texttt{MSE}. One alternative way to measure the distance between two projected vectors is \texttt{MSE}, as employed in the popular non-contrastive SSL algorithm BYOL~\citep{grill2020bootstrap}. When adding region-matching tasks to BYOL and pre-training 50 epochs, \texttt{Softmax} and \texttt{MSE} yield $k$-NN accuracy of 37.2\% and 34.9\%, while the baseline BYOL yields 33.1\%. We also replace the region-matching metric in \shortname{} as \texttt{MSE}, yielding $k$-NN accuracy 72.6\%, which lower than the view-level task only (74.2\%). These results show that  \texttt{Softmax} is essential in $\Lcal_R$.
$(\RN{2})$ Optimal Transport (OT) {\em vs} Simple Argmax. To avoid heavy computational overhead, a simple feature-level argmax solution is considered in Eq. \eqref{eq:obj_region} to pair two local regions. To study the impact of high region-matching quality, we consider OT. Empirically, we observe OT yields slightly higher $k$-NN accuracy at the early stage, but the gain is diminished in the end. Considering the extra computational cost of solving OT with an inner loop in sinkhorn algorithm~\citep{cuturi2013sinkhorn}, we opt for simple argmax in our experiments.   

\begin{table}[t!]
\begin{minipage}[b]{0.54\linewidth}
\centering
\scalebox{0.82}{
\begin{tabular}{ @{\hspace{-0pt}}l@{\hspace{8pt}}|c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c}%rrrrrrrrrrrr
\toprule
 Arch.   &  Objectives & Window S. & Linear & $k$-NN  \\ 
\midrule
\multirow{4}{*}{Swin-T}
& $\Lcal_{V}$ & 7 & 77.0 & 74.2 \\
& $\Lcal_{V}\!+\!\Lcal_{R}$ & 7 &  {\bf 78.1}  &   {\bf 75.7} \\ 
& $\Lcal_{V}$ & 14 & 77.9 & 75.5 \\
& $\Lcal_{V}\!+\!\Lcal_{R}$ & 14 &  {\bf 78.7}  & {\bf 77.0} \\ 
\midrule
\multirow{4}{*}{Swin-S}
& $\Lcal_{V}$ &  7 & 79.2  & 76.8  \\
& $\Lcal_{V}\!+\!\Lcal_{R}$ & 7 &  {\bf 79.5}  & {\bf 77.7}  \\
& $\Lcal_{V}$  & 14 & 79.4  & 77.3  \\
& $\Lcal_{V}\!+\!\Lcal_{R}$ & 14 &   {\bf 80.8}  &  {\bf 79.1}  \\
\midrule
\multirow{4}{*}{Swin-B}
& $\Lcal_{V}$ &  7 & 79.6  & 77.7  \\
& $\Lcal_{V}\!+\!\Lcal_{R}$ & 7 &  {\bf 80.4}  & {\bf 78.9}  \\
& $\Lcal_{V}$ &  14 &  80.5 &   78.3 \\
& $\Lcal_{V}\!+\!\Lcal_{R}$ & 14 &  {\bf 81.3}  & {\bf 79.3}  \\
\bottomrule
\end{tabular} 
}
\vspace{0mm}
    \caption{Ablations of various configurations.}
    \label{tab:cmp_obj}
\end{minipage}\hfill
\begin{minipage}[b]{0.44\linewidth}
\centering
\includegraphics[height=4.5cm]{figs/obj_view_and_region.pdf}
\vspace{-4mm}
\captionof{figure}{Learning curves of different pre-training tasks. For Base model,  $\Lcal_{\text{R}}$ is added from the 200th epoch.}
\label{fig:obj_curves}
\end{minipage}
\vspace{-2mm}
\end{table}


% Note that \shortname{} is a general investigation on multi-stage ViT



\begin{table}[t!]
  \centering
  \centering
  \scalebox{0.83}{
  \begin{tabu}{ll cc | ll | ll}
    \toprule
 \multicolumn{4}{c|}{Pre-training {\bf ResNet50} in different settings}  
   & \multicolumn{2}{c|}{ImageNet-1K}  
   & \multicolumn{2}{c}{COCO}   \\
  Types & Methods &     \#Epochs  & \#Views  &   Linear & $k$-NN & AP$^{bb}$ &  AP$^{mb}$ \\
    \midrule
    \rowfont{\color{gray}}
   & Supervised & & & - & -  &  38.2 & 33.3 \\ \midrule
\multirow{2}{*}{Contrastive}     
   & MoCo-v2 & 200 & 2 & 67.5 & 55.6  & 38.7  & 33.9 \\
   & DenseCL & 200 & 2 & 63.6 {\bf \textcolor{red}{(-3.9)}} & 48.6 {\bf \textcolor{red}{(-7.0)}} & 39.1 {\bf \textcolor{emerald!80}{(+0.4)}}  & 34.2 {\bf \textcolor{emerald!80}{(+0.3)} }\\ \midrule  
\multirow{2}{*}{Non-Contrastive} 
  & $\Lcal_{V}$ & 200 & 2  &   69.2  & 59.9   & 37.8 &  33.1  \\
  & $\Lcal_{V}\!+\!\Lcal_{R}$ & 200 & 2    &  69.9 {\bf\textcolor{emerald!80}{(+0.7)}}  &  61.7 {\bf\textcolor{emerald!80}{(+1.8)}}  &  38.0 {\bf\textcolor{emerald!80}{(+0.2)}}   & 33.2 {\bf\textcolor{emerald!80}{(+0.1)}} \\ 
%  \cline{2-8}  
%   & $\Lcal_{V}$  & 300 & 2+8 &  75.0 &  69.3  &  37.3 & 32.8 \\ 
%   & $\Lcal_{V}\!+\!\Lcal_{R}$   &  300 & 2+8   &  75.7 {\bf\textcolor{emerald!80}{(+0.7)}}   &   71.2 {\bf\textcolor{emerald!80}{(+1.9)} }  & 38.3 {\bf \textcolor{emerald!80}{(+1.0)}}  & 33.5 {\bf\textcolor{emerald!80}{(+0.7)}}   \\ 
    \bottomrule
  \end{tabu}
  }
  \vspace{-2mm}
  \caption{Comparison between contrastive and non-contrastive region-matching tasks.}
  \label{table:region_matching}  
\vspace{-6mm}
\end{table}

\vspace{-2mm}
\subsection{Qualitative Studies}
\vspace{-2mm}

\paragraph{Visualization of correspondences.}  
% \PZ{This item needs to be further polished to impress the reader, instead of to confuse the reader. It seems that Figure 6 (c) improves over Figure 6 (b), but is still worse than Figure 6 (a). Why do we say that "(c) yields higher local region matching similarity scores than (a)"? I guess the score (0.9 > 0.85) is computed by averaging the top-10 correspondence? But is this a reasonable score? We may not want to make the reviewer argue with us on this.} 
% \CL{Good point!  the local matching property of DINO is now considered the target we approximate to}
Given two views of the same image, we use the pre-trained backbone to extract the top-layer features $\zv_1$ and $\zv_2$. 
For each feature vector in $\zv_1$, we find the feature vector in $\zv_2$ that best matches it in terms of highest cosine similarity, as defined in Equation~\eqref{eq:obj_region}. In Figure~\ref{fig:correspondences}, we show the top-10 correspondences between two views for three methods. 
In Figure~\ref{fig:correspondences} (b), 
\shortname{} with $\Lcal_V$ tends to identify pairs in the background as the most matched ones (and in a wrong way in this example). This could be a valid solution to $\Lcal_V$, as the invariance in the level of aggregated global features does not necessarily induce invariances in the local region level. This is significantly alleviated with $\Lcal_R$ (shown in Figure~\ref{fig:correspondences} (c)), a task that implicitly requires local matching. 

Surprisingly, DINO is able to learn good correspondences even without the region-level matching task. To the best of our knowledge, this is a previously unreported intriguing property of self-supervised Transformers with monolithic architectures: good semantic correspondences are automatically learned. We hypothesize that features at lower layers (image patch itself in the extreme case) can directly pass to higher layers, and the former regularizes the latter to remain discriminative. Nevertheless, the proposed $\Lcal_R$ can dramatically reduce the issue, and is good remedy to rescue the loss of semantic correspondence for the multi-stage architecture. 
In Appendix, we quantitatively measures the correspondence learning ability of these SSL methods on ImageNet validation dataset, the observations are consistent: $\Lcal_R$ improves the matching accuracy from 66\% to 91\%.


\begin{figure*}[t!]%\vspace{-25pt}
	\vspace{-0mm}\centering
	\begin{tabular}{c c c}
		\hspace{-2mm}
		\includegraphics[height=2.3cm]{figs/correspondence/pairs_appendix/cute_dog_1_dino.png}  & 
		% \vspace{2mm}
		\hspace{-3mm}
		\includegraphics[height=2.2cm]{figs/correspondence/pairs_appendix/cute_dog_1_lv.png} & 
		\hspace{-3mm}
		\includegraphics[height=2.2cm]{figs/correspondence/pairs_appendix/cute_dog_1_lr.png} 		
		\\
		(a) DINO: DeiT-S  & 
		\hspace{-2mm}
		(b) \shortname{}: $\Lcal_V$    \vspace{2mm} & 
		\hspace{-2mm}		
		(c) \shortname{}: $\Lcal_V\!+\!\Lcal_R$   \hspace{-0mm} \\ 
	\end{tabular}
	\vspace{-3mm}
	\caption{The learned correspondences.  {\bf \textcolor{yellow!80!black}{Yellow}}  lines are the top-10 correspondences between two views, where the numbers indicates the rankings of similarity scores, yellow dots with the same number are paired.
	 }
	\vspace{-3mm}
	\label{fig:correspondences}
\end{figure*}
%  The  {\bf \textcolor{blue!50}{blue}} dot and {\bf \textcolor{red}{red}}  triangle indicates the most similar local regions that correspond to the global feature of the view itself and the other view, respectively.


\begin{figure*}[t!]%\vspace{-25pt}
	\vspace{-0mm}\centering
	\begin{tabular}{c c c c c c c c c}
		\hspace{-3mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/dino/layer11_mask_th0.6_head0.png}  & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/dino/layer11_mask_th0.6_head1.png}  &
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/dino/layer11_mask_th0.6_head2.png}  & 
		\hspace{-2mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lv/mask_th0.6_head_00.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lv/mask_th0.6_head_01.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lv/mask_th0.6_head_02.png} & 
		\hspace{-2mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lr/mask_th0.6_head_00.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lr/mask_th0.6_head_01.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lr/mask_th0.6_head_02.png} 
		\\
		\hspace{-3mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/dino/layer11_mask_th0.6_head3.png}  & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/dino/layer11_mask_th0.6_head4.png}  &
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/dino/layer11_mask_th0.6_head5.png}  & 
		\hspace{-2mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lv/mask_th0.6_head_03.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lv/mask_th0.6_head_04.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lv/mask_th0.6_head_05.png} & 
		\hspace{-2mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lr/mask_th0.6_head_03.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lr/mask_th0.6_head_04.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/cute_dog/esvit_lr/mask_th0.6_head_05.png}
		\\	
		\multicolumn{3}{c}{(a) DINO: DeiT-S} & 
		\multicolumn{3}{c}{(b) \shortname{}: $\Lcal_V$ } & 
		\multicolumn{3}{c}{(c) \shortname{}: $\Lcal_V\!+\!\Lcal_R$ } \\
% 		\multicolumn{3}{c}{(a) DINO: DeiT-S} & 
% 		\hspace{-2mm}
% 		\multicolumn{3}{c}{(b) \shortname{}: $\Lcal_V$ }  & 
% 		\hspace{-2mm}		
% 		\multicolumn{3}{c}{(c) \shortname{}: $\Lcal_V\!+\!\Lcal_R$ } \hspace{-0mm} \\ 
	\end{tabular}
	\vspace{-3mm}
	\caption{Visualization of the the learned attention map for different heads in the last layer. The query is the {\bf \textcolor{blue!50}{blue}} dot in the center of the images. We visualize masks (as {\bf \textcolor{red}{red}}) obtained by thresholding the self-attention maps to
keep 60\% of the probability mass.  Note that all 6 heads are visualized for DINO with DeiT-S, and 6 out of 24 heads in \shortname{} are chosen to visualize (ranked by entropy values). Please see enlarged pictures with all heads in Appendix.
	 }
	\vspace{-5mm}
	\label{fig:attn_vis}
\end{figure*}

% SkyBlue

%
% Lastly, we visualize where the global representation is most similar with in each image views. Both DINO and \shortname{} with $\Lcal_R$ identify the regions closer to foreground objects than  \shortname{} with $\Lcal_V$ only. 




\paragraph{Visualization of attention maps.} We look at the self-attention in the different heads of the last layer in Figure~\ref{fig:attn_vis}. A local region on the edge of the main object is employed as query, and the attended regions are highlighted in red for those the query's top 60\% mass are assigned. In Appendix, we visualize more examples with different query positions.
%
DINO tends to automatically learn class-specific attention maps leading to foreground object segmentation, regardless of its query located in foreground or background. This is probably because main objects remain as the major invariance factor in different augmented views.
This property is lost when a multi-stage architecture is employed, as shown in \shortname{} with $\Lcal_V$. These patterns are consistent for different heads. After introducing $\Lcal_R$ for \shortname{}, we note that the attention maps become more diverse in different heads, \ie entropy values of attentions get more skewed, and attended regions are more different. This is perhaps because  $\Lcal_R$  requires each region to consider many matching tasks to regions in different augmented views, each head automatically learns to distribute the tasks and complete a few of them.



% \begin{itemize}

% \item Variants of efficient transformers: Swin, VIL and CvT.

% \item Pre-training objectives: Instance vs Region. The performance saturation can also be caused by the limited power of the existing instance-based unsupervised frameworks. While these frameworks are currently superior to masked auto-encoding in vision, the underlying instance discrimination task [45] as a pretext task may be too easy to achieve, which may prevent the model from learning stronger representations. To unleash the potential strength of ViT, it may be desired to design more difficult pretext tasks in vision.

% \item Pre-training datasets: ImageNet-1k, ImageNet-22k, WebVision and OpenImages.

% \item Data augmentations: DINO vs DeiT.

% \end{itemize}

\vspace{-3mm}
\section{Conclusions}
\vspace{-3mm}
In this paper, we first discover the automatic correspondence learning property of self-supervised monolithic Transformers. Inspired by this, we present efficient self-supervised vision Transformers (\shortname{}) to with two major insights: a multi-stage Transformer architecture with sparse self-attentions, and a non-contrastive region-matching pre-training task. The synergy of both helps \shortname{} reach the SoTA performance of SSL vision systems with significantly less compute and smaller model size. 
Our study also reveals that exploration of effective solutions to learn from larger and less curated pre-training data in the wild is a key but less studied factor in paving the way toward the scaling success of SSL vision systems.

% A potential future work is to perform self-supervised pre-training for bigger multi-stage ViT models.  Another interesting research direction to investigate the correspondence learning property of self-supervised Transformers for image-text paris, \ie, automatic grounding between regions and words.


\section*{Ethics Statement}
Though self-supervised learning (SSL) has great potentials to learn powerful representation without human annotation, the existing techniques to build SoTA SSL vision systems tend to be {\bf\textcolor{red!100}{Red AI}}~\citep{schwartz2020green}: it could be environmentally unfriendly and the computational cost is extensively high. The required training resource is typically not accessible for a lab environment (thus raising barriers to participation in AI research). For example, the prior art MoCo-v3 has greatly pushes the performance limit of SSL system~\citep{chen2021empirical}. The authors kindly reported that ``it (MoCo-v3, ViT-H) takes 9.8 hours per 100 epochs using 512 TPUs. This is a gigantic scale of training: for the 300-epoch ViT-H, this amounts to $\sim$625 TPU days, or $\sim$1.7 TPU years of training.'' The SoTA model MoCo-v3 with ViT-BN-L/7 should have a higher cost than this. Even for a smaller model ViT-B, ``it takes 24 hours in 128 GPUs (vs. 2.1 hours in 256 TPUs)''. Hence, improving the efficiency of building SoTA SSL systems is of high value for the community and society to achieve {\bf\textcolor{emerald!100}{Green AI}}~\citep{schwartz2020green}.

To this end, we propose \shortname{} to provide more affordable and efficient solutions for the community to experiment and explore the directions of SoTA SSL in computer vision. Our EsViT model shows the best ImageNet linear probe performance compared with all existing SSL vision systems, and is 3.5$\times$ parameter-efficient and has 10$\times$ higher throughput than previous SoTA. This efficiency gain can significantly decrease its carbon footprint and increase its inclusivity, encouraging more researchers to participate the study of the SSL topic. 


\section*{Reproducibility Statement}
Our paper provides comprehensive empirical studies on the \shortname{} algorithm. 
We provide PyTorch-style pseudo-code in Appendix. We also include an example code with instruction as supplementary material to ensure the reproducibility. 
For empirical results on both various network architecture and large-scale datasets, we provide detailed hyper-parameter specifications.
We will release the pre-trained checkpoints and codebase for the research community for reproducible research.


==> subtex/main_nips_submission.tex <==
\maketitle

\begin{abstract}
  This paper investigates efficient self-supervised vision transformers (\shortname{}) for visual representation learning. The first empirical study is presented on multi-stage ViT architectures for self-supervised learning. 
  Our study reveals two insights towards building \shortname{}:
  1) Multi-stage architectures with sparse self-attentions can greatly reduce complexity, but lacks correspondences between regions.
  2) A region matching pre-training task is proposed to improve the efficiency and boost learned representations significantly.
We show that the synergy of both in \shortname{} achieves 81.1\% top-1 on the ImageNet linear probe evaluation, with around an order magnitude of higher throughput, compared with prior arts of comparable accuracy.  When transferring to downstream linear classification tasks, \shortname{} outperforms its supervised counterpart on 17 out of 18 datasets.
The code and models will be publicly available.   

%   \JG{Do you position the paper as an empirical study or to propose a new method -- EsViT? If it is both, then clarify that ``we first present an empirical study..., Then, we propose a new region-level pre-training task (MPP) inspired by MLM for language model pre-training to significantly improve the efficiency of SSL of vision transformers, leading to new SoTA results on...''}
  

\end{abstract}

%   Region-mixed data augmentations help when added in the late stage of pre-training.

\section{Introduction}
\vspace{-2mm}
Self-supervised learning (SSL) with Transformers~\cite{vaswani2017attention} has become a de facto standard of model choice in natural language processing (NLP). The dominant approaches such as GPT~\citep{radford2018improving} and BERT~\citep{devlin2019bert} are pre-training on a large text corpus and then fine-tuning to various smaller task-specific datasets, showing superior performance. Larger Transformers pre-trained with larger-scale language datasets often lead to a stronger generalization ability, demonstrated by improved performance in downsteam tasks (with no sign of performance saturation yet), as exemplified in GPT-3~\citep{brown2020language}. 

In computer vision (CV), however, self-supervised visual representation learning is still dominated by convolutional neural networks (CNNs). Sharing a similar goal/spirit with NLP, SSL in CV aims to learn general-purpose image features from raw pixels without relying on manual supervisions, and the learned networks serve as the backbone of various downstream tasks such as classification, detection and segmentation. Recently, impressive performance have been achieved by CNN-based SSL, outperforming state-of-the-art (SoTA) fully-supervised pre-training methods~\citep{he2020momentum,caron2020unsupervised} on tasks with a limited number of labels. The key to success is contrastive learning: maximizing agreement of learned representations between differently augmented views of the same example.  Recent works, including SimCLR-v2~\citep{chen2020big}, BYOL~\citep{grill2020bootstrap} and SwAV~\cite{caron2020unsupervised}, have scaled up the model of CNN-based contrastive learning to millions of parameters.  However, a large performance gap remains for CNN-based SSL in CV, compared to the scaling successes of Transformer in NLP.
 
% and is becoming the building block in many computer vision applications. 

% The pre-trained model produces general-purpose features and serve as the backbone of various downstream tasks such as classification, detection and segmentation, improving the generalization of those task-specific models that are often trained on limited amounts of task labels. 

Several attempts have been made to close the gap by combining SSL with self-attention architectures. Early works include Selfie~\citep{trinh2019selfie}, which generalizes the concept of masked language modeling of BERT for images. The idea has been recently revisited in Vision Transformer (ViT)~\citep{dosovitskiy2020image} via pre-training on a much larger scale dataset, \eg JFT-300M.  ImageGPT (iGPT)~\citep{chen2020generative} generalizes the concept of auto-regressive language modeling of GPT for images, showing encouraging ImageNet recognition accuracy with a large model size. Contrastive learning with ViT has also been studied very recently in DINO~\citep{caron2021emerging} and MoCo-v3~\citep{chen2021empirical}, where new SoTA result by  linear probe evaluation on ImageNet-1K is achieved, by exhaustively consuming computation resource on full self-attention operators with long sequences of splited image patches.

% \begin{wrapfigure}{R}{0.45\textwidth}
% \vspace{-5mm}
% \begin{minipage}{0.55\textwidth}
% \scriptsize
% \centering
% \hspace{-3mm}
% \includegraphics[height=5.2cm]{figs/ssl_sota_tradeoff.pdf}
% \vspace{-1mm}
% \caption{\small Comparison under the linear classification protocol
% on ImageNet. All are reported as unsupervised pre-training on the ImageNet-1M training set, followed by supervised linear classification trained on frozen features, evaluated on the validation set. The parameter counts are those of the feature extractors.} 
% \label{fig:ssl_sota_curves}
% \vspace{-2mm}
% \end{minipage}
% \end{wrapfigure}


\begin{figure*}[t!]%\vspace{-25pt}
	\vspace{-0mm}\centering
	\begin{tabular}{c c}
		\hspace{-4mm}
		\includegraphics[height=4.55cm]{figs/ssl_sota_tradeoff_throughput.pdf}  & 
		% \vspace{2mm}
		\hspace{-0mm}
		\includegraphics[height=4.6cm]{figs/ssl_sota_param.pdf} \\
% 		(a) Proposed multi-stage architecture \vspace{2mm} & 
% 		\hspace{-6mm}
% 		(b) Baseline monolithic architecture \hspace{-0mm} \\ 
	\end{tabular}
	\vspace{-3mm}
	\caption{Efficiency vs accuracy comparison under the linear classification protocol on ImageNet. Left: Throughput of all SoTA SSL vision systems, circle sizes indicates model parameter counts; Right: performance over varied parameter counts for models with moderate (throughout/\#parameters) ratio. Please refer Section~\ref{sec:imagenet_probe} for details.
	 }
	\vspace{-3mm}
	\label{fig:hero_cmp}
\end{figure*}

% 	 \footnote{MoCo-v3 ViT/7 and DINO DeiT/8 are excluded when comparing model size, as they requires much higher compute complexity per parameter count than others, shown in Table~\ref{tab:main_result_cls}. }



Aiming to improve the {\em efficiency} of Transformer-based SSL, this paper presents {\em {\bf E}fficient {\bf s}elf-superivsed {\bf Vi}sion {\bf T}ransformers} (\shortname{}), by considering a multi-stage architecture and a region-based pre-training task for unsupervised representation learning. Our main findings and contributions can be summarized as follows:

\begin{minipage}{1.0\textwidth}
\centering



\begin{itemize}[leftmargin=5.5mm]
\item  We present the first comprehensive empirical study of multi-stage vision Transformer architectures for SSL. Though greatly reducing complexity, we find that this multi-stage architecture causes the loss of semantic correspondence between local regions, an intriguing property of self-supervised Transformers that is previously unreported. A region matching task is proposed to alleviate this issue, and further improve the learned representations and attentions.

\item \shortname{} significantly reduces the cost in building SoTA SSL vision systems, as summarized in Figure 1, and shows better scaling performance on accuracy vs. throughput and model size.
Under the linear evaluation protocol, \shortname{} achieves 80.8\% top-1 accuracy, approaching SoTA (81.0\%, MoCo-v3 with ViT-BN-L/7~\citep{chen2021empirical}) with  $6\times$ less parameters and $22\times$ higher throughput, and outperforms the 2nd place method (80.1\%, DINO with ViT-B/6~\citep{caron2021emerging}), with $1.5\times$  less parameters and $6\times$ higher throughput.

\item Compared with its supervised counterpart Swin Transformers~\citep{liu2021Swin}, \shortname{} shows superior performance on 17 out 18 datasets, when transferring the learned representations to downstream linear classification tasks. 

\end{itemize}

\end{minipage}



% ~\CL{To do in the end}
% We further investigate the impact of pre-training datasets and data augmentations, to set a solid baseline for future research in efficient Transformer-based SSL.
%

% $(\RN{1})$ 
% $(\RN{2})$ 
% $(\RN{3})$
% $(\RN{4})$



% The multi-stage architectures enable the first Transformer-based SSL backbone for dense visual prediction tasks.

\vspace{-1mm}
\section{Methods}
\vspace{-3mm}

\paragraph{Background.} An overview of existing Transformer-based SSL methods is illustrated in Figure~\ref{fig:illustration_esvit}(a). They are emerged very recently to lead the state-of-the-art performance on the ImageNet linear probe task~\citep{chen2021empirical,caron2021emerging}. It inherits the successes from (1) monolithic Transformer architectures that dominate in NLP~\citep{devlin2019bert,radford2018improving}, and (2) instance-level contrastive learning objectives that demonstrate arguably the best SSL performance in computer vision~\citep{chen2020simple}.
As common practice, different crops of each image are taken under random data augmentation. Each augmented view is partitioned into non-overlapped patches with patch size $P\!\times\!P$. Concatenating a $\texttt{[CLS]}$ token (as a global token) with these patches,  they are encoded by a stack of Transformer layers with the same network configurations, such as ViT~\citep{dosovitskiy2020image} or DeiT~\citep{touvron2020training}. Hence, the input sequence and output representation share the same number of tokens, and it is clear that each local patch has its unique corresponding top-layer feature representation. The global representation of different views are further projected into a latent space using a shared MLP head, where the agreement among views is maximized.

Though simple and effective, the existing Transformer-based SSL methods require a large amount of compute resources to reach SoTA performance. To strike for a better balance between accuracy and efficiency, we present \shortname{}, by considering a multi-stage architecture and a region-based pre-training task, described next.

\subsection{Network Architectures: From Monolithic to Multi-stage ViT Backbone}
Inspired by great successes of the multi-stage ConvNet architecture such as VGG~\citep{simonyan2014very}/ResNets~\citep{he2016deep} for computer vision, the multi-stage Transformer-based networks have been explored very recently in the supervised learning setting~\citep{vaswani2021scaling,wang2021pyramid,liu2021Swin,zhang2021vil,wu2021cvt}. 
This paper presents the first empirical study of multi-stage Transformer architectures for SSL. Though straightforward in implementation, changing from monolithic to multi-stage architecture without careful treatments may lose some %attractive
desirable properties of self-supervised Transformers, as discussed later.

\paragraph{Multi-stage ViT.} An overview of the multi-stage Transformer architecture is shown in Figure~\ref{fig:illustration_esvit} (b). Each stage consists of a {\em patch merging/embedding} module, and an {\em efficient Transformer} module.
$(\RN{1})$ The patch merging module plays a slightly different role in different stages. In the first stage, it splits an input RGB image into non-overlapping
patches. Each patch is treated as a ``token'', constructed as a concatenation of the raw pixel RGB values, which is further projected into a $C$-dimension feature.
In the later stage, the patch merging module concatenates the features of each group of $2\times2$ neighboring patches, and applies a linear layer on the 4$C$-dimensional concatenated features. This reduces the number of tokens by a multiple of $2\times2=4$, and the output dimension is set to $2C$.
$(\RN{2})$ An efficient transformer module with multiple Transformer blocks are then employed to enable interactions among the merged features. 
The two modules above are repeated for multiple times, typically 4 times, resulting in a multi-stage ViT. As a result, a hierarchical representation is generated: the number of tokens is reduced and the feature dimension (and the number of heads in self-attentions) of each token is increased, as the network
gets deeper. 
% Please see Figure~\ref{fig:illustration_esvit} (b) for a brief illustration of this concept.


\begin{figure*}[t!]%\vspace{-25pt}
	\vspace{-0mm}\centering
	\begin{tabular}{c c}
		\hspace{-4mm}
		\includegraphics[height=5.1cm]{figs/esvit1.pdf}  & 
		% \vspace{2mm}
		\hspace{-0mm}
		\includegraphics[height=5.1cm]{figs/esvit2.pdf} \\
		(a) Baseline monolithic architecture \vspace{2mm} & 
		\hspace{-6mm}
		(b) Proposed multi-stage architecture \hspace{-0mm} \\ 
	\end{tabular}
	\vspace{-3mm}
	\caption{Architecture comparison. (a) The traditional monolithic transformer architecture.  For all layers, the transformer blocks share the same network configurations and input token sequence sizes are the same. (b) The multi-stage Transformer architecture organizes an input image into a long sequence of smaller patches, sparse self-attentions are utilized at early stages to maintain model expressiveness while reducing computational complexity; The neighboring tokens at an intermediate layer are gradually merged, constituting a short sequence to ease the compute burden of self-attention at late stages.
	 }
	\vspace{-3mm}
	\label{fig:illustration_esvit}
\end{figure*}

\paragraph{Efficient Transformers.} Since a larger number of patches is often produced at the early stages, an efficient Transformer with sparse self-attentions is considered to reduce the computational complexity. The basic idea is to split the feature maps into non-overlapping local windows (with size $W\!\times \!W$), and self-attention is performed within each local window. This however has one drawback that features in different local windows cannot interact. Various methods have been proposed to best approximate full-attention among all features, with different trade-off between accuracy and efficiency.


%
We briefly describe three schemes as follows, and benchmark them in the experiments.
$(\RN{1})$ 
{\em Swin Transformer}~\citep{liu2021Swin}: A shifted window partitioning approach is proposed, which alternates between two partitioning configurations in consecutive Transformer blocks, so that each local feature is grouped into different windows in self-attentions.
$(\RN{2})$
{\em Vision Longformer (ViL)}~\citep{zhang2021vil}: Features in each local window are further allowed to attend all features in the 8-neighboring windows.
$(\RN{3})$
{\em  Convolution vision Transformer (CvT)}~\citep{wu2021cvt}: Features in neighboring windows are considered in the convolutional projection in self-attentions. Please refer each paper for detailed description.

\paragraph{Relative Position Bias.} To facilitate SSL, we consider relative position bias~\citep{liu2021Swin} to characterize the spatial information between features for the three efficient Transformers aforementioned, and do not use absolute position embeddings. % if used. 
This is because augmented views of varied resolutions can be cropped from anywhere in an image in SSL,  maintaining the relative positions is easy in implementation, and is largely sufficient for invariance learning among these views. 

% In computing self-attention, we follow  by including a relative position bias $B \in \R^{M2xM2}$ to each head in computing similarity: Since the relative position along each axis lies in the range $[-M+1, M-1]$, we parameterize a smaller-sized bias matrix $\hat{B} \in \R^{(2M-1) \times (2M-1)}$, and values in B are taken from $\hat{\Bmat}$.


\subsection{Pre-training Tasks: Delving into Views with Regions}

We build our SSL systems on top of the recent method {\em self-distillation with no labels} (DINO)~\citep{caron2021emerging}.
Knowledge distillation is a learning paradigm where a student network $g_{\thetav_s}$ is trained
to match the output of a given teacher network $g_{\thetav_t}$
, parameterized by $\thetav_s$ and $\thetav_t$ respectively. 
The neural network $g$ is composed of a backbone $f$ (\eg Transformers or ConvNets), and of a projection head $h$: $g = h \circ f$. The features used in downstream tasks are the output of backbone $f$.
%
In SSL, different augmented views $\Tilde{\xv}$ of an image $\xv$ are fed into backbone network to obtain feature maps $\zv =f(\Tilde{\xv})$. An MLP head combined with \text{softmax} further converts the feature vector $z \in \zv$ into probability $p=h(z)$. DINO updates teacher and student network alternatively:
%
$(\RN{1})$ Given a fixed teacher network, the student network is updated by minimizing the cross-entropy loss:
% $\thetav_s  \leftarrow \min_{\thetav_s} \Mcal (s, t) = - p_t \log p_s $.
$\thetav_s  \leftarrow \arg \min_{\thetav_s} \Mcal(s, t ; \thetav_s)$, where $\Mcal(s, t) = - p_t \log p_s$.
%
$(\RN{2})$ The teacher model is updated as an exponential moving average (EMA) on the student weights
$\thetav_t  \leftarrow \lambda \thetav_t + (1 - \lambda) \thetav_s$, with $\lambda$  following a cosine schedule
from 0.996 to 1 during training. Please refer to \citep{caron2021emerging} for details.


More precisely, from a given image, we generate a set $\Vcal$ of different views following~\citep{caron2021emerging}. This set contains views of two different resolutions $\Vcal = [\Vcal_g, \Vcal_l  ]$, where $\Vcal_g = \{ \Tilde{\xv}_{g_i} | i=1,2 \}$ is a global-view set of higher resolution, and $\Vcal_l = \{ \Tilde{\xv}_{l_i} | i=1,\dots,8 \}$  is a local-view set of lower resolution. All views $\Vcal$  are passed through the student while only the global views $\Vcal_g$ are passed through the teacher.
%
The resulting feature map at the top layer for each view is $\zv = [z_1, \dots, z_T] $, where $T$ is the sequence length, and $z_i$ is a region-level representation for the local patch at position $i$. Average pooling is applied to obtain the view-level representation $\bar{z}= \text{avg-pool} (\zv)$.  


\paragraph{View-level task}
Given the augmented view set for student $ \Vcal$ and teacher $ \Vcal^*$, a set of pairs $ \Pcal = \{ (s,t) | \Tilde{\xv}_s \in \Vcal,  \Tilde{\xv}_t \in \Vcal^*  \text{~and~} s \neq t $ \} is constructed to perform cross-view prediction tasks. We consider the pre-training task at the view level proposed by~\citep{caron2021emerging}:
%
\begin{align}\label{eq:obj_view}
\Lcal_V = \frac{1}{| \Pcal|} \sum_{ (s, t) \in \Pcal }  
\Mcal_V ( s, t), ~~\text{with} ~~
 \Mcal_V (s, t ) = -  p_{s} \log p_t,
\end{align}
%
where 
$p_s = h(\bar{z}_s)$ and $p_t = h(\bar{z}_t)$ are the probability output of an MLP head $h$ over the view-level representations $\bar{z}_s$ and $\bar{z}_t$, learned by student and teacher, respectively. In DINO, ViT/DeiT are considered, hence the view-level representation is the feature of the $\texttt{[CLS]}$ token.

\paragraph{Region-level task}
The $\Lcal_{V}$ above encourages ``local-to-global'' correspondences only at a coarse level: the large crop and the small crop are matched in the view level, leaving region-to-region correspondence unspecified. 
Inspired by the success of masked language modeling task in BERT, it is important to have region-level pre-training task for computer vision, so that the model can take into account the co-occurrences/structures between local features. Unfortunately, directly performing masked patch
prediction (MPP) for the multi-stage Transformer architecture is infeasible, as the one-to-one correspondences between the input visual tokens and output features get diluted due to the merging operation. Even for monolithic architectures, MPP has not been proved effective in computer vision, as empirically shown in~\citep{dosovitskiy2020image}.

% \JG{This ``background'' reviews existing work. Now, you may start a new section to describe the proposed method EsViT, which uses the proposed region-level task for pre-training.}

To address this problem, we propose an effective, dense self-supervised learning method
that directly works at the level of local features
by taking into account their correspondences:
%
\begin{align}\label{eq:obj_region}
\vspace{-2mm}
& \Lcal_R = \frac{1}{| \Pcal|}  \sum_{ (s, t) \in \Pcal }  
\Mcal_R ( s, t), ~~\text{with} ~~
 \Mcal_R (s, t ) = - \frac{1}{T}\sum_{i=1}^T  p_{j^*} \log p_i, ~~ j^* = \arg \max_{j} \frac{z_i^T z_j}{\|z_i\| \|z_j\|},
\end{align}
where 
$p_i = h^{\prime}(z_i)$ and $p_j = h^{\prime}(z_j)$ are the probability outputs of a new MLP head $h^{\prime}$ over the local features of student $z_i \in \zv_s$ and teacher $z_j \in \zv_t$, respectively. $j^*$ is the index of the feature in $\zv_t$ that best matches the $i$-th feature in $\zv_s$, in the sense of highest cosine similarity. 

We can consider $\Lcal_R$ as a proxy to mimick masked language modeling in BERT, where the ``ground-truth'' local token is a soft label provided by the teacher network, while the student network makes predictions to match that target, based on the context of regions in a different augmented view.
Though the ideas of leveraging local-level pre-training tasks have been explored for ConvNets in the context of contrastive learning in a bid to improve dense visual prediction tasks~\citep{xiong2020loco,wang2020dense}, our $\Lcal_R$ is different in that no negative samples/queue is needed, we find that $\Lcal_R$ is particularly effective in improving Transformers and their learned attentions, as demonstrated in our experiments. 

%
\begin{wrapfigure}{R}{0.5\textwidth}
\vspace{-5mm}
\begin{minipage}{0.5\textwidth}
\scriptsize
\centering
\hspace{-3mm}
\includegraphics[height=3.2cm]{figs/esvit_preidctions.pdf}
\vspace{-1mm}
\caption{Pre-training objectives.} 
\label{fig:esvit_preidctions}
\vspace{-3mm}
\end{minipage}
\end{wrapfigure}
%
The overall pre-training objective of \shortname{} is $\Lcal = \Lcal_R + \Lcal_V$ (show in Figure~\ref{fig:esvit_preidctions}), we learn to match the feature distributions at both the view and region levels by minimizing the cross-entropy loss w.r.t. the parameters of the student network $g_{\thetav_s}$. By default, the full objective is used from the beginning. One can also load a checkpoint trained by $\Lcal_V$ only, and add $\Lcal_R$ for continual pre-training, which is shown effective in boosting performance in our experiments.
%
Note that applying $\Lcal_R$ on the traditional monolithic Transformer architecture can be prohibitively computationally expensive, as it requires $\Ocal(T^2)$ to compute $\Lcal_R$. For a typical image of resolution $224 \!\times \!224$, the feature map length  of ViT/DeiT (with patch size 16) at the top layer is $T=196$, while the multi-stage architecture yields $T=49$, which requires 3 times less compute in computing $\Lcal_R$.






% \subsection{Data Augmentation: Region-Mixed Views}

\vspace{-2mm}
\section{Related Works}
\vspace{-2mm}
\paragraph{Self-supervised ConvNets.}
ConvNets-based SSL have been extensively studied in the literature. Based on the pre-training tasks, they can broadly categorized into three classes:  Handcrafted pretext tasks~\cite{doersch2015unsupervised,noroozi2016unsupervised,pathak2016context,gidaris2018unsupervised,zhang2016colorful,larsson2016learning,zhang2017split,pu2016variational,donahue2019large}, contrastive learning~\cite{dosovitskiy2015discriminative,zhuang2019local,oord2018representation,hjelm2018learning,bachman2019learning,he2020momentum,chen2020simple,grill2020bootstrap} and prototype learning~\cite{caron2018deepcluster,caron2020unsupervised,li2020prototypical,xie2016unsupervised,yang2016joint,ji2019invariant,zhan2020online}. 
It is also known that data augmentations play a crucial role in SSL pipeline~\cite{chen2020improved,caron2020unsupervised,tian2020makes,li2020self}. 
The impact of pre-training dataset size/quality is explored for ConvNets in SSL~\citep{goyal2021self,tian2021dnc}.
To date, the search of best pre-taining tasks/datasets and augmentations are based on CNNs. Among them, SimCLR-v2~\citep{chen2020big}, BYOL~\citep{grill2020bootstrap} and SwAV~\cite{caron2020unsupervised} achieve the highest ImageNet linear probe performance with large ConvNet architectures. The performance tends to saturate with an increasingly growing model size, raising a question if ConvNets reach a limit in SSL. 





\paragraph{Self-supervised vision Transformers.} The research on Transformer-based self-supervised representation learning just scratches the tip of the iceberg, and only a few attempts are made on this topic.  ImageGPT~\citep{chen2020generative} and MoCo-v3~\citep{chen2021empirical} dedicate huge compute resource with large models to exploring the frontier. 
DINO~\citep{caron2021emerging} achieves comparable performance of large self-supervised ConvNets using small/medium-size Transformers. The proposed \shortname{} further pursue efficient solutions to self-supervised vision Transformers.


\paragraph{Transformers for vision.} Vision Transformers (ViT)~\citep{dosovitskiy2020image} shows the great potentials of generalizing Transformers for computer vision, by achieving compelling accuracy in supervised learning, especially with large-scale data and high capacity models. DeiT~\citep{touvron2020training} further provides an effective ViT training strategy to ease the adaption of Transformers for practitioners.
Transformers have also been applied to other vision tasks, ranging from low-level tasks such as image generation~\cite{parmar2018image,chen2020generative} and enhancement~\cite{chen2020pre,yang2020learning}, to high-level tasks such as  object detection~\cite{carion2020end,zhu2020deformable,zheng2020end,dai2020up} and segmentation~\cite{wang2020max,wang2020end}, and to vision-language tasks~\cite{lu2019vilbert,tan2019lxmert,chen2019uniter,su2019vl,li2019visualbert,li2019unicoder,zhou2019unified,li2020oscar}.
%
Marrying Transformers with multi-stage architectures~\citep{vaswani2021scaling,wang2021pyramid,liu2021Swin,zhang2021vil,wu2021cvt} show higher classification accuracy in supervised learning, and enables applicability of Transformers for a broader range of vision tasks.
Given these properties, we believe multi-stage ViT is a must-study baseline for SSL in computer vision.

% DeiT~\citep{touvron2020training}, 
% Swin Transformer~\citep{liu2021Swin}, 
% Vision Longformer (ViL)~\citep{zhang2021vil}, 
% Convolutions vision Transformers (CvT)~\citep{wu2021cvt}, 
% Pyramid vision Transformer (PvT)~\citep{wang2021pyramid}
% ViT~\citep{dosovitskiy2020image}


% Note that footnotes are properly typeset \emph{after} punctuation marks.\footnote{As in this example.}



\begin{table}[t!]
\footnotesize % \small
\centering

\begin{tabular}{ @{\hspace{-0pt}}l@{\hspace{8pt}}c@{\hspace{2pt}}@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c}%rrrrrrrrrrrr
\toprule
 Method   &  \#Parameters $\downarrow$~~ &  Throughput (Image/s) $\uparrow$ & Linear $\uparrow$~~ & $k$-NN $\uparrow$  \\ 
\hline
\multicolumn{3}{l}{\em \hspace{-3mm} SoTA SSL methods with Big ConvNets}  & & \\
SwAV, RN50w5~\citep{caron2020unsupervised} & 586 & 76 & 78.5 &  67.1 \\
BYOL, RN200w2~\citep{grill2020bootstrap} & 250 & 123 & 79.6 & 73.9 \\
SimCLR-v2, RN152w3+SK ~\citep{chen2020big} & 794 & 46 & 79.8 & 73.1 \\
\midrule
\multicolumn{3}{l}{\em \hspace{-3mm} Skyline methods with excessively long sequences for self-attentions}  & & \\
DINO, DeiT-S/8~\citep{caron2021emerging} & 21 & 180 & 79.7 & 78.3 \\
DINO, ViT-B/8~\citep{caron2021emerging} & 85 & 63 & 80.1 & 77.4 \\
MoCo-v3, ViT-B-BN/7~\citep{chen2021empirical} & 85 & $\sim$63 & 79.5 & - \\
MoCo-v3, ViT-L-BN/7~\citep{chen2021empirical} & 304 & $\sim$17 & 81.0 & - \\
iGPT, iGPT-XL~\citep{chen2020generative} &  6801 & - & 72.0 & - \\
\rowcolor{Gray}
\shortname{}, Swin-S/$W\!=\!14$ & 49 & 383   &  80.8   &   79.1 \\
\rowcolor{Gray}
\shortname{}, Swin-B/$W\!=\!14$ & 87 & 254   &  {\bf 81.1}   &  {\bf 79.2} \\
\midrule
\multicolumn{3}{l}{\em \hspace{-3mm} Transformer-based SSL, with moderate sequence length for self-attentions}  & & \\
\textcolor{gray}{Masked Patch Pred., ViT-B/16~\citep{dosovitskiy2020image}} & \textcolor{gray}{85} & \textcolor{gray}{312} &  ~\textcolor{gray}{79.9}$^{\dagger}$ & - \\
DINO, DeiT-S/16~\citep{caron2021emerging} & 21 & 1007 & 77.0 & 74.5 \\
DINO, ViT-B/16~\citep{caron2021emerging} & 85 & 312 & 78.2 & 76.1 \\
MoCo-v3, ViT-B/16~\citep{chen2021empirical} &  85  & 312 & 76.7 & - \\
MoCo-v3, ViT-H-BN/16~\citep{chen2021empirical} & 632 & $\sim$32 & 79.1 & - \\
MoBY, Swin-T~\citep{xie2021moby} & 28 &  808 & 75.1 & - \\
\rowcolor{Gray}
\shortname{}, Swin-T & 28 &  808 &  78.1  & 75.7 \\
\rowcolor{Gray}
\shortname{}, Swin-S & 49 &  467 &  79.5  & 77.7 \\
\rowcolor{Gray}
\shortname{}, Swin-B & 87 &  297 &  {\bf 80.4}  & {\bf 78.9} \\
\bottomrule
\end{tabular} \\

% \rowfont{\color{gray}}

\vspace{2mm}
\caption{Comparison with SoTA across different architectures on ImageNet linear probing. ViT-BN is ViT that has BatchNorm~\citep{frankle2020training}, and “$/P$” denotes a patch size of $P\!\times\!P$. ``$\sim$'' indicates through-puts estimated by comparing different papers, detailed in Appendix. $^{\dagger}$ The mask patch prediction in~\citep{dosovitskiy2020image} is pre-trained on JFT-300M and end-to-end fine-tuned in ImageNet, which we append as a reference.}
\label{tab:main_result_cls}
\vspace{-5mm}
\end{table}




% \begin{table}[t!]
% \footnotesize % \small
% \centering

% \begin{tabular}{ @{\hspace{-0pt}}l@{\hspace{8pt}}|c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c}%rrrrrrrrrrrr
% \toprule
%  Arch.   &  Objectives & Window & Linear & $k$-NN  \\ 

% \hline
% \multirow{3}{*}{Swin-Tiny}
% & $f_{V}$ & 7 & 77.0 & 74.2 \\
% & $f_{V}$ & 14 & 77.9 & 75.5 \\
% & $f_{V}+f_{R}$ & 7 &  78.1  &  75.7 \\
% & $f_{V}+f_{R}$ & 14 &  {\bf 78.7}  & {\bf 77.0} \\
% \midrule
% \multirow{3}{*}{Swin-Small}
% & $f_{V}$ &  7 & 79.2  & 76.8  \\
% & $f_{V}$  & 14 &   &    \\
% & $f_{V}+f_{R}$ & 7 &  {\bf 79.5}  & {\bf 77.7}  \\
% & $f_{V}+f_{R}$ & 14 &     &    \\
% \bottomrule
% \end{tabular} \\

% \vspace{2mm}
% \caption{Ablations of pre-training tasks and window sizes.}
% \label{tab:cmp_obj}
% \vspace{-0mm}
% \end{table}


% \begin{figure*}[h!]%\vspace{-25pt}
% \vspace{-0mm}\centering 
% \centering
% \hspace{-3mm}
% \includegraphics[height=3.9cm]{figs/obj_view_and_region.pdf}
% \vspace{-1mm}
% \caption{Learning curves of different objectives.} 
% \label{fig:obj_curves}
% \vspace{-3mm}
% \end{figure*}

\vspace{-3mm}
\section{Experimental Results}
\vspace{-3mm}
We study unsupervised pre-training performed in ImageNet-1K dataset~\citep{deng2009imagenet} without labels. The default training details are described as follows, mostly following~\citep{caron2021emerging}. We train with the Adamw optimizer~\citep{loshchilov2018fixing}, a batch size of $512$, and and total epochs $300$. Linear warmup of the learning rate is used during the first 10 epochs, with its base value determined with the linear scaling rule~\citep{goyal2017accurate}: $lr = 0.0005*\text{batchsize}/256$. After this warmup, the learning rate is decayed with a cosine schedule. 
%
We build our systems based on Swin Transformers in our experiments.  
%
Swin-B has a model size and computation complexity similar to ViT-B/DeiT-B (patch size 16). We also considered Swin-T and Swin-S, which have the complexity that are similar to those of ResNet-50 (DeiT-S) and ResNet-101, respectively. The default window size is $W\!=\!7$.

\vspace{-3mm}
\subsection{Comparisons with Prior Art on ImageNet}
\label{sec:imagenet_probe}
\vspace{-3mm}
One major common protocol to evaluate SSL is linear probe on ImageNet-1K, where features are extracted from a frozen backbone, and a supervised linear classifier is trained. For all Transformer models, we use the concatenation of view-level features $\bar{z}$ in the last 4 layers (the results are similar to the use of last 3 or 5 layers in our initial experiments). We report top-1 and $k$-NN classification accuracy  on the ImageNet validation set.
%
Table~\ref{tab:main_result_cls} presents comparisons with all SoTA SSL vision systems across various network architectures. Please refer to Figure~\ref{fig:hero_cmp} for visual comparisons over scaling parameter counts and throughput. Our main findings are summarized below.

\paragraph{Comparisons with self-supervised Transformers.} 

Both iGPT~\citep{chen2020generative} and the masked patch prediction in~\citep{dosovitskiy2020image} are earlier variants of masked auto-encoding schemes, mimicking the behaviors of GPT~\citep{radford2018improving} and BERT~\citep{devlin2019bert} in NLP, respectively. The DINO- and MoCo-based ViT has higher accuracy and smaller models than iGPT, under the same linear probing protocol and training data. At the similar level of model size and compute complexity, the proposed \shortname{} improve SoTA methods DINO/MoCo-v3 by a large margin: \shortname{} (Swin-B) outperforms  DINO (ViT-B/16) by 2.2\% linear probe accuracy and 2.8\% $k$-NN accuracy in absolute values.
\shortname{} (Swin-B) even performs slightly better than DINO (ViT-B/8) (0.3\% higher linear probe accuracy and 1.5\% higher $k$-NN accuracy), with $4\times$ higher throughput.
MoBY~\citep{xie2021moby} is a con-current work that investigates multi-stage ViT in SSL. With the same architecture Swin-T, our \shortname{} pre-training tasks significantly outperform MoBY, showing 3\% higher accuracy. Overall, the proposed \shortname{} shows the best performance compared with all systems, except that it is slightly worse than MoCo-v3 built with ViT-L-BN/7, which has $6\times$ more model parameters and is $22\times$ slower. Due to limited resources, we leave the study of further scaling \shortname{} as future work.

% \CL{ToDO, where to put?} Our self-supervised model \shortname{} has larger improvement gaps when the models are bigger than the supervised results in~\citep{liu2021Swin}. For example, from Swin-S to Swin-B, \shortname{} shows an accuracy improvement of 0.9\%, while supervised learning shows 0.3\%  improvement when trained in ImageNet-1K.



\paragraph{Comparisons with big ConvNets.}
We compare with the SoTA big ResNets reported by SimCLR-v2~\citep{chen2020big}, BYOL~\citep{grill2020bootstrap} and SwAV~\cite{caron2020unsupervised}. Among them, the best accuracy $79.8\%$ under the linear probing protocol is reported by SimCLR-v2 with SK-ResNet, where Selective Kernel (SK)~\citep{li2019selective} is a form of attention to enhance CNNs. 
It is clear in Figure~\ref{fig:hero_cmp} (b) that all ConvNets-based SSL methods show an envelope in the regime of scaling up model sizes after passing $500$M.
\shortname{} achieves better accuracy than their highest envelope, with $16\times$ less model parameters and $8\times$ higher throughput.

\paragraph{Longer sequences for self-attentions.} It is observed that using longer sequences in self-attentions can improve recognition accuracy: In iGPT~\citep{chen2020generative} sequence length is increased in the pixel domain; DINO and MoCo-v3 explore longer sequences by reducing the patch size to $8\times8$ or $7\times7$ (``/8'' or``/7'' in Figure~\ref{fig:hero_cmp} and Table~\ref{tab:main_result_cls}), respectively. This keeps the model parameter counts unchanged, but dramatically increases compute complexity (measured by increased FLOPs and decreased throughput), \eg to around $6\times$ reported in MoCo-v3. 
% This reveals that small patches provide gains.
In \shortname{}, longer sequences in self-attention is implemented by increasing the window size. We experiment this by considering a window size of $W\!=\!14$, and report the results in Table~\ref{tab:cmp_obj}, where we see a consistent accuracy improvement of around 1-2\%. In Table~\ref{tab:main_result_cls}, \shortname{} with Swin-S/$W\!=\!14$  achieves highest 79.1\% $k$-NN accuracy, and comparable linear probe accuracy with SoTA, with almost an order of magnitude higher efficiency.  




\begin{table}[t!]
\begin{minipage}[b]{0.54\linewidth}
\centering
\begin{tabular}{ @{\hspace{-0pt}}l@{\hspace{8pt}}|c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c}%rrrrrrrrrrrr
\toprule
 Arch.   &  Objectives & Window S. & Linear & $k$-NN  \\ 
\midrule
\multirow{4}{*}{Swin-T}
& $\Lcal_{V}$ & 7 & 77.0 & 74.2 \\
& $\Lcal_{V}\!+\!\Lcal_{R}$ & 7 &  {\bf 78.1}  &   {\bf 75.7} \\ 
& $\Lcal_{V}$ & 14 & 77.9 & 75.5 \\
& $\Lcal_{V}\!+\!\Lcal_{R}$ & 14 &  {\bf 78.7}  & {\bf 77.0} \\ 
\midrule
\multirow{4}{*}{Swin-S}
& $\Lcal_{V}$ &  7 & 79.2  & 76.8  \\
& $\Lcal_{V}\!+\!\Lcal_{R}$ & 7 &  {\bf 79.5}  & {\bf 77.7}  \\
& $\Lcal_{V}$  & 14 & 79.4  & 77.3  \\
& $\Lcal_{V}\!+\!\Lcal_{R}$ & 14 &   {\bf 80.8}  &  {\bf 79.1}  \\
\midrule
\multirow{2}{*}{Swin-B}
& $\Lcal_{V}$ &  7 & 79.6  & 77.7  \\
& $\Lcal_{V}\!+\!\Lcal_{R}$ & 7 &  {\bf 80.4}  & {\bf 78.9}  \\
\bottomrule
\end{tabular} 
\vspace{2mm}
    \caption{Ablations of pre-train tasks and window sizes.}
    \label{tab:cmp_obj}
\end{minipage}\hfill
\begin{minipage}[b]{0.44\linewidth}
\centering
\includegraphics[height=4.5cm]{figs/obj_view_and_region.pdf}
\captionof{figure}{Learning curve of different pre-training tasks. For Base model,  $\Lcal_{\text{R}}$ is added from the 200th epoch.}
\label{fig:obj_curves}
\end{minipage}
\vspace{-4mm}
\end{table}

\paragraph{Ablation: The effectiveness of $\Lcal_R$.} We compare the pre-training objective with and without $\Lcal_R$ in Table~\ref{tab:cmp_obj}. Across different model scales and window sizes, the proposed region level $\Lcal_R$ can consistently improve the performance. The gains can be clearly seen by $k$-NN accuracy (around 1-2\%),  where no additional tuning is needed as in linear probe. Figure~\ref{fig:obj_curves} demonstrates that $\Lcal_R$ helps model convergence, and can be used as a drop-in to improve models trained with the view level task.


\begin{wraptable}{r}{7.9cm}
% \begin{table}[t!]
\footnotesize % \small
\centering
\vspace{-5mm}
\begin{tabular}{ @{\hspace{8pt}}c@{\hspace{2pt}}@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}|c@{\hspace{5pt}}c@{\hspace{5pt}}|c@{\hspace{5pt}}c}%rrrrrrrrrrrr
\toprule
\multirow{2}{*}{Method}    &  \multirow{2}{*}{\#Param.}  &   \multirow{2}{*}{ Im./s} & \multicolumn{2}{c|}{100 epochs}   &  \multicolumn{2}{c}{300 epochs}  \\ 
   &  &  & Linear & $k$-NN & Linear & $k$-NN \\ 
\hline
DeiT & 21 &  1007 & 73.1  &  69.0 & 75.9  &  73.2 \\ %  \cline{2-6}
Swin & 28 &  808 & 75.3  &   70.0 & 77.1 &  73.7 \\
ViL & 28 &  386   &  75.4 & 70.1 & 77.3 &  73.9 \\
CvT & 29 &  848  &  75.5 &  70.6 & 77.6  & 74.8  \\
% \midrule
% \multirow{4}{*}{300}
%  & DeiT & 21 &  1007 & 75.9  &  73.2 \\ \cline{2-6}
%  & Swin & 28 &  808 & 77.1 &  73.7 \\
%  & ViL & 28 &  386 & 77.3 &  73.9 \\
%  & CvT & 29 &  848 & 77.6  & 74.8  \\
\bottomrule
\end{tabular} \\
%
\vspace{0mm}
\caption{Different sparse attentions in \shortname{}.}
\label{tab:cmp_attn}
\vspace{-5mm}
\end{wraptable}



\paragraph{Ablation: Comparison of sparse attentions.} We investigate different efficient sparse Transformers in Table~\ref{tab:cmp_attn}. DeiT is shown as a baseline reference. Batch size = 1024 in this experiment. To ensure fair comparison, we modify all into a 4-stage architecture with the number of Transformer layers in each stage as 2-2-6-2. ViL and CvT can be safely used as alternatives to Swin, and could potentially achieve better performance. Due to limited resources, we choose to scale up Swin in our experiments first to study the limit of \shortname{}, leave the scaling of others as future work.

% Note that \shortname{} is a general investigation on multi-stage ViT


\subsection{Transfer Learning}
We also conduct transfer learning in downstream tasks to evaluate the quality of learned representations. Two sets of tasks are considered:


\begin{minipage}{0.99\textwidth}
\centering

\begin{itemize}[leftmargin=5.5mm]
\item {\em Classification on a suite of 18 small datasets}. As exemplified in \citep{radford2021learning}, it is a common and clean approach to evaluate a learned representation by fitting a linear classifier on
the representation and measuring its performance across multiple datasets.  We study 18 datasets used in~\citep{radford2021learning}. Automatic hyper-parameter tuning is considered to ensure fairness of comparison. Besides averaged $\texttt{scores}$, we report $\texttt{\#\!\! wins}$ as the number of datasets on which the model outperforms its supervised counterpart. Detailed dataset description and settings are in Appendix.
\end{itemize}

\end{minipage}

\begin{minipage}{0.99\textwidth}
\centering

\begin{itemize}[leftmargin=5.5mm]
\item {\em Detection and segmentation on COCO}. Different from previous monolithic self-supervised ViT, the multi-stage architecture in \shortname{} can be readily used for dense visual tasks that require hierarchical feature representations.
\end{itemize}

\end{minipage}


\paragraph{Comparison with supervised learning counterparts.} We compare with the supervised-learning Swin, whose checkpoints are downloaded from the official codebase\footnote{\url{https://github.com/microsoft/Swin-Transformer}}. 
Figure~\ref{fig:esvit_transfer_cls} shows the classification results of Swin-S, \shortname{} consistently outperforms its supervised variant, often by a large margin. Similar conclusions are drawn for other model sizes. On COCO detection and segmentation task, however, comparable results with the supervised counterpart are obtained, as shown in Table~\ref{table:coco_res} for Swin-T.



\begin{figure*}[t!]%\vspace{-25pt}
\vspace{-0mm}\centering 
\centering
\hspace{-3mm}
\includegraphics[height=3.9cm]{figs/transfer_cls_swin_small.pdf}
\vspace{-1mm}
\caption{Transfer learning to a wide variety of datasets. Fitting a linear
classifier on \shortname{}’s features outperforms using its supervised  counterpart on 17 out of 18 datasets.} 
\label{fig:esvit_transfer_cls}
\vspace{-2mm}
\end{figure*}


\paragraph{Effects of larger, less-curated pre-train datasets.}
The performance of Transformer-based SSL research has thus far been limited to highly curated pre-train data such as ImageNet-1K. To push the frontier in leveraging large amounts of unlabeled data, we explore the effects of pre-training from larger, less-curated image datasets:  
WebVision-v1~\citep{li2017webvision}, OpenImages-v4~\citep{kuznetsova2020open} and ImageNet-22K~\citep{deng2009imagenet}, described in Appendix. The pre-train epochs on different datasets are adjusted so that all models see a similar number of augmented views. 
We summarize the results in Table~\ref{table:datasets_res} and would like to emphasize the following findings.
% We find there is indeed a large difference in the resulting representation quality.
First, all \shortname{} pre-trained checkpoints outperform supervised checkpoint in downstream classification tasks, but performance varies a lot, with ImageNet-22K checkpoint showing the best transfer ability. Second, ImageNet-1K pre-trained model shows the best ImageNet-1K linear probe performance. 
We hypothesize that it is not only the size of pre-train dataset matters, but also the distribution of image classes matters: more diverse and well-balanced distribution results in a stronger generalization ability. Similar observations are reported in a concurrent work~\citep{tian2021dnc} for ConvNets.





\begin{table}[t!]
\begin{minipage}[b]{0.43\linewidth}

  \centering
  \scalebox{0.92}{
  \begin{tabu}{l |  lll }
    \toprule
   & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$   \\ \cline{2-4}
   % \midrule
    \rowfont{\color{gray}}
    Supervised &  46.0 & 68.1 & 50.3   \\
    \shortname{}  & 46.2 & 68.0 & 50.6   \\
    \midrule
   &  AP$^{mb}$ & AP$^{mb}_{50}$ & AP$^{mb}_{75}$  \\ \cline{2-4}
    % \midrule
    \rowfont{\color{gray}}
    Supervised & 41.6 & 65.1 & 44.9  \\
    \shortname{} & 41.6 & 64.9 & 44.8  \\
    \bottomrule
  \end{tabu}
  }
  \vspace{2mm}
  \caption{COCO Detection \& Segmentation.}
  \label{table:coco_res}  
\end{minipage}\hfill
\begin{minipage}[b]{0.57\linewidth}
  \centering
  \scalebox{0.83}{
  \begin{tabu}{l | cc | cc}
    \toprule
    Pre-train Data    
    &   \multicolumn{2}{c|}{ImageNet-1K}  
    & \multicolumn{2}{c}{18 Datasets}    \\
          &   Linear & $k$-NN & Scores & \# Wins \\
    \midrule
    \rowfont{\color{gray}}
    Supervised & - & -  &  77.29 & - \\
    ImageNet-1K &  77.1 & 73.7  & 80.66  & 16 \\
    WebVision-v1    & 75.4 &  69.4 & 80.00 & 14 \\ 
    OpenImages-v4    & 69.6 &  60.3   & 77.97 & 10 \\
    ImageNet-22K   & 73.5 & 66.1  & {\bf 81.03} & {\bf 17} \\    
    \bottomrule
  \end{tabu}
  }
  \vspace{2mm}
  \caption{Impact of the pre-train datasets.}
  \label{table:datasets_res}  
\end{minipage}
\vspace{-6mm}
\end{table}



% \begin{table}
%   \centering
%   \scalebox{0.80}{
%   \begin{tabu}{l | cc | llllll| cc}
%     \toprule
%     Pre-train     
%     &   \multicolumn{2}{c|}{ImageNet-1K}  
%     &  \multicolumn{6}{c|}{  COCO Detection  \& Segmentation} & \multicolumn{2}{c}{Classification on 18 Datasets}    \\
%           &   Linear & $k$-NN  & AP$^{bb}$ & AP$^{bb}_{50}$ & AP$^{bb}_{75}$  &  AP$^{mb}$ & AP$^{mb}_{50}$ & AP$^{mb}_{75}$  & Scores & \# Wins \\
%     \midrule
%     \rowfont{\color{gray}}
%     Supervised & - & - &  46.0 & 68.1 & 50.3  & 41.6 & 65.1 & 44.9   &  77.29 & - \\
%     ImageNet-1K &  77.1 & 73.7  & 46.2 & 68.0 & 50.6 & 41.6 & 64.9 & 44.8 & 80.66  & 16 \\
%     WebVision-v1    & 75.4 &  69.4 &   &  &  &   & & & 80.00 & 14 \\ 
%     OpenImages-v4    & 69.6 &  60.3  & 46.0 &  67.6 & 50.6 & 41.3 & 64.5 & 44.1 & 77.97 & 10 \\
%     ImageNet-22K   & 73.1 & 66.1 & 46.0 & 67.9 & 50.8  &  41.6 & 64.9 & 44.7  & {\bf 81.03} & {\bf 17} \\    
%     \bottomrule
%   \end{tabu}
%   }
%   \vspace{2mm}
%   \caption{Impact of the pre-training datasets for \shortname{} in transfer learning.  The supervised Swin-T checkpoint is downloaded from the official codebase.}
%   \label{table:coco}  
% \end{table}






\subsection{Qualitative Studies}


\begin{figure*}[t!]%\vspace{-25pt}
	\vspace{-0mm}\centering
	\begin{tabular}{c c c}
		\hspace{-2mm}
		\includegraphics[height=2.2cm]{figs/correspondence/dino_correspondence.png}  & 
		% \vspace{2mm}
		\hspace{-3mm}
		\includegraphics[height=2.2cm]{figs/correspondence/lv_correspondence.png} & 
		\hspace{-3mm}
		\includegraphics[height=2.2cm]{figs/correspondence/lr_correspondence.png} 		
		\\
		(a) DINO: DeiT-S ($r=0.85$) & 
		\hspace{-2mm}
		(b) \shortname{}: $\Lcal_V$ ($r=0.63$)   \vspace{2mm} & 
		\hspace{-2mm}		
		(c) \shortname{}: $\Lcal_V\!+\!\Lcal_R$ ($r=0.90$)  \hspace{-0mm} \\ 
	\end{tabular}
	\vspace{-3mm}
	\caption{The learned correspondences.  {\bf \textcolor{yellow!80!black}{Yellow}}  lines are the top-10 correspondences between two views. $r$ is the threshold on the similarity. The  {\bf \textcolor{blue!50}{blue}} dot and {\bf \textcolor{red}{red}}  triangle indicates the most similar local regions that correspond to the global feature of the view itself and the other view, respectively.
	 }
	\vspace{-1mm}
	\label{fig:correspondences}
\end{figure*}



\begin{figure*}[t!]%\vspace{-25pt}
	\vspace{-0mm}\centering
	\begin{tabular}{c c c c c c c c c}
		\hspace{-3mm}
		\includegraphics[height=1.43cm]{figs/attn/dino/layer11_mask_th0.6_head0.png}  & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/dino/layer11_mask_th0.6_head1.png}  &
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/dino/layer11_mask_th0.6_head2.png}  & 
		\hspace{-2mm}
		\includegraphics[height=1.43cm]{figs/attn/lv/mask_th0.6_head0.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/lv/mask_th0.6_head1.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/lv/mask_th0.6_head2.png} & 
		\hspace{-2mm}
		\includegraphics[height=1.43cm]{figs/attn/lr/mask_th0.6_head1.png} &
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/lr/mask_th0.6_head2.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/lr/mask_th0.6_head3.png} 
		\\
		\hspace{-3mm}
		\includegraphics[height=1.43cm]{figs/attn/dino/layer11_mask_th0.6_head3.png}  & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/dino/layer11_mask_th0.6_head4.png}  &
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/dino/layer11_mask_th0.6_head5.png}  & 
		\hspace{-2mm}
		\includegraphics[height=1.43cm]{figs/attn/lv/mask_th0.6_head13.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/lv/mask_th0.6_head14.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/lv/mask_th0.6_head15.png} & 
		\hspace{-2mm}
		\includegraphics[height=1.43cm]{figs/attn/lr/mask_th0.6_head11.png} &
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/lr/mask_th0.6_head12.png} & 
		\hspace{-4mm}
		\includegraphics[height=1.43cm]{figs/attn/lr/mask_th0.6_head14.png} 
		\\	
		\multicolumn{3}{c}{(a) DINO: DeiT-S} & 
		\multicolumn{3}{c}{(b) \shortname{}: $\Lcal_V$ } & 
		\multicolumn{3}{c}{(c) \shortname{}: $\Lcal_V\!+\!\Lcal_R$ } \\
% 		\multicolumn{3}{c}{(a) DINO: DeiT-S} & 
% 		\hspace{-2mm}
% 		\multicolumn{3}{c}{(b) \shortname{}: $\Lcal_V$ }  & 
% 		\hspace{-2mm}		
% 		\multicolumn{3}{c}{(c) \shortname{}: $\Lcal_V\!+\!\Lcal_R$ } \hspace{-0mm} \\ 
	\end{tabular}
	\vspace{-0mm}
	\caption{Visualization of the the learned attention map for different heads in the last layer. The query is the {\bf \textcolor{blue!50}{blue}} dot in the center of the images. We visualize masks (as {\bf \textcolor{red}{red}}) obtained by thresholding the self-attention maps to
keep 60\% of the probability mass.  Note that all 6 heads are visualized for DINO with DeiT-S, and 6 out of 24 heads in \shortname{} are randomly chosen to visualize. Please see enlarged pictures with all heads in Appendix.
	 }
	\vspace{-3mm}
	\label{fig:attn_vis}
\end{figure*}

% SkyBlue

\paragraph{Visualization of correspondences.}  
% \PZ{This item needs to be further polished to impress the reader, instead of to confuse the reader. It seems that Figure 6 (c) improves over Figure 6 (b), but is still worse than Figure 6 (a). Why do we say that "(c) yields higher local region matching similarity scores than (a)"? I guess the score (0.9 > 0.85) is computed by averaging the top-10 correspondence? But is this a reasonable score? We may not want to make the reviewer argue with us on this.} 
% \CL{Good point!  the local matching property of DINO is now considered the target we approximate to}
Given two views of the same image, we use the pre-trained backbone to extract the top-layer features $\zv_1$ and $\zv_2$. 
For each feature vector in $\zv_1$, we find the feature vector in $\zv_2$ that best matches it in terms of highest cosine similarity, as defined in Equation~\eqref{eq:obj_region}. We consider there is a solid match between two regions if the highest similarity is larger than a given threshold $r$ (\ie $s > r$). In Figure~\ref{fig:correspondences}, we show the top-10 solid correspondences between two views for three methods. 
In Figure~\ref{fig:correspondences} (b), 
\shortname{} with $\Lcal_V$  tends to assign most regions in View 1 to one single region in View 2. This could be a valid solution to $\Lcal_V$, as the invariance in the level of aggregated global features does not necessarily induce invariances in the local region level. This is significantly alleviated with $\Lcal_R$ (shown in Figure~\ref{fig:correspondences} (c)), a task that implicitly requires local matching. 

Surprisingly, DINO is able to learn good correspondences even without the region-level matching task. To the best of our knowledge, this is a previously unreported intriguing property of self-supervised Transformers with monolithic architectures: good semantic correspondences are automatically learned. We hypothesize that features at lower layers (image patch itself in the extreme case) can directly pass to higher layers, and the former regularizes the latter to remain discriminative. Nevertheless, the proposed $\Lcal_R$ yields comparable local region matching similarity scores with DINO, and is good remedy to rescue the loss of semantic correspondence for the multi-stage architecture. 
%
Lastly, we visualize where the global representation is most similar with in each image views. Both DINO and \shortname{} with $\Lcal_R$ identify the regions closer to foreground objects than  \shortname{} with $\Lcal_V$ only.




\paragraph{Visualization of attention maps.} We look at the self-attention in the different heads of the last layer in Figure~\ref{fig:attn_vis}. A local region on the main object is employed as query, and the attended regions are highlighted in red for those the query's top 60\% mass are assigned .
%
DINO tends to automatically learns class-specific attention maps leading to foreground object segmentations, while \shortname{} with $\Lcal_V$ attend broadly on the images. These patterns are consistent for different heads. After introducing $\Lcal_R$ for \shortname{}, we note that the attention maps become much sparser in each head, and more diverse across different heads. This is perhaps because  $\Lcal_R$  requires each region to consider many matching tasks to regions in different augmented views, each head automatically learns to distribute the tasks and complete a few of them.



% \begin{itemize}

% \item Variants of efficient transformers: Swin, VIL and CvT.

% \item Pre-training objectives: Instance vs Region. The performance saturation can also be caused by the limited power of the existing instance-based unsupervised frameworks. While these frameworks are currently superior to masked auto-encoding in vision, the underlying instance discrimination task [45] as a pretext task may be too easy to achieve, which may prevent the model from learning stronger representations. To unleash the potential strength of ViT, it may be desired to design more difficult pretext tasks in vision.

% \item Pre-training datasets: ImageNet-1k, ImageNet-22k, WebVision and OpenImages.

% \item Data augmentations: DINO vs DeiT.

% \end{itemize}

\vspace{-3mm}
\section{Conclusions}
\vspace{-3mm}
In this paper, we present efficient self-supervised vision Transformers (\shortname{}) with two major insights: a multi-stage Transformer architecture with sparse self-attentions, and a region-matching pre-training task. The synergy of both helps \shortname{} reach the comparable if not better performance of SoTA SSL vision systems with significantly less compute and model size.
A potential future work is to perform self-supervised pre-training for bigger multi-stage ViT models. Our study also reveals that exploration of effective solutions to learn from larger and less curated pre-training data is a key but less studied factor in paving the way toward the scaling success of SSL vision systems. 

